Robustness of Online Inventory Balancing to Inventory Shocks

In classic adversarial online resource allocation problems such as AdWords, customers arrive online while products are given offline with a fixed initial inventory. To ensure revenue guarantees under uncertainty, the decision maker must balance consumption across products. Based on this, the prevalent policy "inventory balancing (IB)" has proved to be optimal or near-optimal competitive in almost all classic settings. However, these models do not capture various forms of inventory shocks on the supply side, which play an important role in real-world online assortment and can significantly impact the revenue performance of the IB algorithm. Motivated by this paradigm, we introduce a variant of online assortment planning with inventory shocks. Our model considers adversarial exogenous shocks (where supply increases unpredictably) and allocation-coupled endogenous shocks (where an inventory reduction is triggered by the algorithms and re-adjusted after a usage duration), whose combination leads to non-monotonic inventory fluctuations. As our main result, we show the robustness of IB-type strategies against such shocks by designing a new family of optimal competitive algorithms called "Batched Inventory Balancing (BIB)." Using a novel randomized primal-dual method, we bound the competitive ratio of BIB against optimal offline. We show that with proper choice of a certain parameter, this competitive ratio is asymptotically optimal and converges to (1-1/e) as initial inventories grow, in contrast to the original IB which no longer achieves the optimal ratio in this new model. Moreover, we characterize BIB's competitive ratio parametric by its penalty function and show that it matches exactly the competitive ratio of IB without shocks. Our refined analysis reduces the dual construction to a combinatorial "interval assignment problem" whose algorithmic solution may be of independent interest.

==> Paper/EIBB.tex <==
\label{sec:EIBB}
As mentioned earlier in the introduction, we aim to use the primal-dual analysis to prove \Cref{thm:concave competitive ratio}. In contrast to prior work that used a similar approach, we have two main technical challenges to solve:
(i) different units of the same product 
require different dual assignments (since the time they are added to the inventory due to exogenous shock 
might be different),
and
(ii)
inventory level of an arbitrary 
bin is not decreasing anymore due to both endogenous and exogenous shock, which turned out to be a crucial property needed in prior primal-dual analyses for matching and assortment. 

\paragraph{Overview of the analysis} To address challenge (i), we come up with a dual
construction at the unit level (not at the product level) that depends on which bin the unit belongs.
To address challenge (ii), roughly speaking, 
the dual construction incorporates randomness in a specific fashion. To do so, it uses a transformed version of inventory levels of allocatable bins using a particular mapping. 
For exponential penalty function the mapping is easy. For the general concave penalty functions, the mapping is combinatorial and the final dual construction is rather involved; 
it uses a chain of techniques to reduce the problem 
of finding an appropriate dual assignment 
to solving a sub-problem called  
\emph{interval assignment problem}.  
We defer the details of this reduction 
and how to solve this sub-problem to 
\Cref{sec:IBB proof}. 
Instead, here we prove a weaker version
(i.e., \Cref{thm:exponential competitive ratio})
for the special case of 
exponential penalty function $\exponential$.

% The competitive ratio of EBIB in \Cref{thm:exponential competitive ratio} does not depend
% on rental duration or fee of any of the products. It is asymptotically
% tight in sense that no online algorithm can obtain a competitive ratio better than $(1 - \sfrac{1}{e})$ even if there is no replenishment and resources are non-reusable \citep[cf.][]{GNR-14}. However, it is strictly worse than that of \cref


\subsubsection{Proof of \Cref{thm:exponential competitive ratio}}
	Recall that $\batchid$ is the bin to which 
	unit $k$ of product $i$ belongs.
	    	We denote $\cnt_{i,t}$ by the value of bin counter $\cnt_i$
	immediately after possible update of $\cnt_i$
	due to exogenous shock at time $t$ (i.e., step-8 in BIB).
	By construction, for any bin $j\leq \cnt_{i,t}-1$
	and unit $k$ 
	such that $(i, k) \in \batch_{i}^j$, 
	we have 
	$\addtime(i, k) \leq t$.\footnote{Also, for any bin $\batch_{i}^{j}$ in BIB, we have $\cnt_{i, t}\leq j$
			if $t <
						\max_{k\in \batch_{i}^{j}}
			\addtime(i,k)$, and $\cnt_{i, t}=j+1$ if $t = \max_{k\in \batch_{i}^{j}}\addtime(i,k)$.}
	
			
			Fix any time $t$ and
			any product $i$. Given the current set of bins $\batch_{i}^j$ for $j\in[1:\cnt_{i,t}]$, we can define ``adjusted bins'' as follows:\footnote{Loosely speaking, by introducing the adjusted bins, we can amortize the revenue gains from the ``ready'' bins in the BIB algorithm to the dual assignments for units in both ``ready'' bins and ``batching'' bin. }
			\begin{align*}
			\batchTilde_{i}^1 &\triangleq \batch_{i}^1
			\cup \batch_{i}^2[\gamma\inventory_i]\\
			\batchTilde_{i}^j &\triangleq \batch_{i}^j
			\ \backslash\  \batch_{i}^j[\gamma\inventory_i]
			\cup \batch_{i}^{j+1}[\gamma\inventory_i]
			~~~~
			\text{for all $j\in[2:\cnt_{i,t}-1]$}
			\end{align*}
			where $\batch_{i}^{j}[\gamma\inventory_i]$
			is the set of the first
			$\gamma\inventory_i$ units 
			added into $\batch_{i}^{j}$.
			See \Cref{fig:binTilde structure}
			for a graphical illustration of 
			$\batchTilde_{i}^{j}$.
			By construction, 
			$\cup_{j=1}^{\cnt_{i, t}-1}
			\batchTilde_{i}^{j}$ contains 
			all units 
			of product $i$ that
			are added to inventory due to 
			exogenous shock
			no later than $t$.
% 			\begin{figure}
%     \centering
%     \input{Paper/figs/fig-binTilde-structure}
%     \caption{
%     The construction of adjusted bins $\batchTilde_i^j$ used in the dual assignments given the original bins.}
%     \label{fig:binTilde structure}
% \end{figure}
			We also define $\batchidTilde$ to be the index of the adjusted bin that unit $k$ belongs to (i.e., 
			$k\in
			\batchTilde_{i}^{\batchidTilde}$). Moreover, define
			adjusted arrival time $\addtimeTilde(i,k)\triangleq
			\max_{k'\in \batch_{i}^{\batchidTilde}}
			\addtime(i,k')$
			and 
			$\indexsetTilde(t) = 
			\cup_{\assortment \in \assortmentspace}
			\left(\prod_{i\in \assortment}
			\{(i,k):\addtimeTilde(i,k)\leq t\}
			\right)$.
			Note that $\addtimeTilde(i, k) \leq \addtime(i,k)$
			and $\indexset(t)\subseteq 
			\indexsetTilde(t)$
			for all $i, k, t$. Note also that for any adjusted bin with index ${j}>1$, $\addtimeTilde(i, k)$ for any unit $k$ in this adjusted bin is essentially the arrival time of the last non-charging unit in this set.
			
			Now, consider 
			the following modified linear program
			\ref{eq:exante-adversarial-relax}.
	\begin{align}
\label{eq:exante-adversarial-relax}
\tag{$
\EARPrime
% {
% \{\choice_t, \repleni\}_{i\in[n],t\in[\totaltime]}
% }
$}
	\begin{array}{llll}
	{\max
	\limits_{\mathbf \alloc \geq \mathbf 0}}~~&
	\displaystyle\sum\nolimits_{t=1}^\totaltime 
	\displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(t)}
	\displaystyle\sum\nolimits_{i=1}^n
	\reward_i\choice_t(\indexnew, i) \curalloc
	&\text{s.t.}& \\[1em]
	  &
	\displaystyle\sum\nolimits_{\tpre = t}^{
 \totaltime,\wedge t+\duration_i-1
 % \totaltime\land t + \duration_i - 1
 }
	\displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(\tpre):
	(i, k)\in \indexnew}
	\choice_{\tpre}(\indexnew, i)
	\prealloc \leq 1
	& i \in [n],\ 
	k\in[\finalinventoryi],\
	t \in [\addtimeTilde(i, k): \totaltime]&
	\\[1em]
	&
	\displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(t)}
	\curalloc 
	\leq 1
	&t \in [\totaltime]&
\end{array}
\end{align}
By construction, \ref{eq:exante-adversarial-relax}
can be interpreted as an instance
where every 
unit $k$ of product $i$ are added due to exogenous shock 
earlier, i.e., decreasing from 
$\addtime(i, k)$ to $\addtimeTilde(i, k)$.
Hence, it
is an upper bound of 
ex ante relaxation
\ref{eq:exante-adversarial}.
We formalize this upper bound in \Cref{lem:tilde relaxation} and defer its proof to \Cref{apx:tilde relaxation}.


\begin{restatable}{lemma}{tilderelax}
\label{lem:tilde relaxation}
    For any sequence 
    $
	\{\choice_t, \repleni\}_{i\in[n],t\in[\totaltime]}$,
	the optimal objective value of\ \ref{eq:exante-adversarial}
	is at most the optimal objective value of 
	\ref{eq:exante-adversarial-relax}.
\end{restatable}
\begin{comment}
\begin{proof}
    Consider any feasible solution 
    $\{\curalloc\}_{
    t\in[\totaltime],\indexnew \in \indexset(t)}$
    in \ref{eq:exante-adversarial}, and let
    $\{\curalloc\primed\}_{
    t\in[\totaltime],\indexnew \in \indexsetTilde(t)}$
    be:
    $\curalloc\primed = \curalloc$ if $\indexnew\in \indexset(t)$, and 
    $\curalloc\primed = 0$ otherwise.
    % \begin{align*}
    %     \curalloc\primed = \left\{
    %     \begin{array}{cc}
    %       \curalloc    & \text{if $\indexnew \in \indexset(t)$} \\
    %        0  & \text{otherwise}
    %     \end{array}
    %     \right.
    % \end{align*}
    Note that 
    $\{\curalloc\primed\}_{
    t\in[\totaltime],\indexnew \in \indexsetTilde(t)}$ is
    feasible in \ref{eq:exante-adversarial-relax},
    and its objective value equals 
    the objective value of $\{\curalloc\}_{
    t\in[\totaltime],\indexnew \in \indexset(t)}$
    in \ref{eq:exante-adversarial}. So the optimal value of \ref{eq:exante-adversarial-relax} is no smaller than \ref{eq:exante-adversarial}, as desired.
\end{proof}
\end{comment}


In the proof of \Cref{thm:exponential competitive ratio},
we construct a randomized dual assignment for
\ref{eq:exante-adversarial-relax}
	that is only feasible in expectation. 
	Interestingly, this is enough for our 
	analysis because of the following technical lemma.\footnote{In \citet{DJK-13}, the authors utilize \Cref{lem:random primal-dual} to construct a randomized dual assignment where the randomness comes from the algorithm. In contrast, in our analysis, the randomness is due to the nature, i.e., consumers' choices.}

\begin{lemma}[\citet{DJK-13}]
	\label{lem:random primal-dual}
	Suppose a randomized primal-dual algorithm constructs a feasible primal assignment with value $P$ 
	(which is a random variable) and
	a dual assignment (not necessarily feasible) with value
	$D$ (which is also a random variable), such that
	% \begin{enumerate}
		% \item 
  (i) for some  constant $\Gamma$, it always holds that $P \geq \Gamma\cdot D$~,
			% 
		% \item 
  (ii) the expectations of the randomized dual assignments form a feasible dual solution.
	% \end{enumerate}
Then, the expectation of $P$ is at least $\Gamma \cdot {\OPT}$ where $\OPT$ is the value of the optimum solution.
\end{lemma}

\begin{comment}

We are now ready to present our primal-dual analysis for the simpler case of EBIB. 
\begin{proof}
[Proof of \Cref{thm:exponential competitive ratio}]
	Consider the following primal linear program 
	\ref{eq:exante-adversarial-relax}, and its dual program with dual variables $\{\inventoryduali\}$ 
	and $\{\probduali\}$ defined as follows:
	% \begin{align*}
	% \begin{array}{llll}
	% {\max
	% \limits_{\mathbf \alloc \geq \mathbf 0}}~&
	% \displaystyle\sum\nolimits_{t=1}^\totaltime 
	% \displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(t)}
	% \displaystyle\sum\nolimits_{i=1}^n
	% \reward_i\choice_t(\indexnew, i) \curalloc
	% &\text{s.t.}& \\[1em]
	%   \langle\theta_{i,k, t}\rangle
	%   &
	% \displaystyle\sum\nolimits_{\tpre = t}^{\min\{\totaltime,t+\duration_i-1\}}
	% \displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(\tpre):
	% (i, k)\in \indexnew}
	% \choice_{\tpre}(\indexnew, i)
	% \prealloc \leq 1
	% & i \in [n],\ 
	% k\in[\finalinventoryi],\
	% t \in [\addtimeTilde(i, k): \totaltime]&
	% \\[1em]
	%   \langle\lambda_{t}\rangle
	% &
	% \displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(t)}
	% \curalloc 
	% \leq 1
	% &t \in [\totaltime]&\\
	% \intertext{We then construct its dual program with dual variables $\{\inventoryduali\}$ 
	% and $\{\probduali\}$ as follows:} 
		
  \begin{align*}
	\begin{array}{llll}
  \min
		\limits_{\boldsymbol{\theta},\boldsymbol{\lambda} \geq \mathbf 0} &
		\displaystyle\sum\nolimits%\limits
		_{i=1}^n
		\displaystyle\sum\nolimits%\limits
		_{k=1}^{\finalinventoryi}
		\displaystyle\sum\nolimits%\limits
		_{t=\addtimeTilde(i,k)}^\totaltime
		\inventoryduali
		+
		\displaystyle\sum\nolimits_{t =1}^\totaltime
		\probduali
		& 
		\text{s.t.} 
		&\\ 
	  \langle\curalloc\rangle
		&
		\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}\geq \displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\reward_i\choice_t(\indexnew, i)
		& t \in [\totaltime],\ \indexnew \in \indexsetTilde(t)
		\vspace{1mm}
		% \\
		% &
		% \qquad\qquad\qquad\qquad
		% \qquad\qquad
		% \geq \displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		% \reward_i\choice_t(\indexnew, i)
		% & t \in [\totaltime],\ \indexnew \in \indexsetTilde(t)
		% &
	\end{array}
\end{align*}	
	Let $\indexnew_t$ be the unit-specified assortment offered to consumer $t$.
	Recall $\curinventoryi$ 
	is the 
	inventory level of bin $j$ of  product $i$ at time period $t$ 
	before 
	the realization of 
	consumer $t$'s randomized choice.
% 	and $\batchid$ is the bin to which 
% 	unit $k$ of product $i$ belongs.
% 	    	We denote $\cnt_{i,t}$ by the value of bin counter $\cnt_i$
% 	immediately after possible update of $\cnt_i$
% 	due to replenishment at time $t$ (i.e., step-8 in BIB).
% 	By construction, for any bin $j\leq \cnt_{i,t}-1$,
% 	and unit $k$ s.t.\ $(i, k) \in \batch_{i, j}$, we have 
% 	$\addtime(i, k) \leq t$.
    Consider the following assignments of primal (which is deterministic) and 
    % $\{\probduali\}$ in 
    dual (which is randomized):
	\begin{align*}
		&\textit{Primal:} &\curalloc &= \indicator{\indexnew_t = \indexnew},\\
		&\textit{Dual:} &\probduali &= 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		\reward_i 
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchid}}
    {|\batch_{i}^{\batchid}|}
		\right) 
			\cdot
			\indicator{\text{a unit 
			from $\batch_{i}^{\batchid}$
			is selected at time $t$}} \\
			& &\inventoryduali &= 
			\reward_i\left(
			\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
			\right) -
			\pen\left(
\frac{\curinventory_{i,t}^{\batchidTilde}, -1}
    {|\batch_{i}^{\batchidTilde}|}
			\right)
			\right) \cdot
			\indicator{\text{a unit 
			from $\batch_{i}^{\batchidTilde}$
			is selected at time $t$}}~.
	\end{align*}
	where 
		$\indicator{\cdot}$ is an indicator operator. 
		Note that product $i$ is selected at time $t$ 
		if it belongs to the unit-specified assortment 
		set $\indexnew_t$ 
		and 
		consumer arriving at time $t$ chooses this product.  
% 		
% 		Fix any time $t$ and
% 			any product $i$, we define 
% 			\begin{align*}
% 			\batchTilde_{i,1} &= \batch_{i,1}
% 			\cup \batch_{i,2}[\gamma\inventory_i]\\
% 			\batchTilde_{i,j} &= \batch_{i,j}
% 			\ \backslash\  \batch_{i,j}[\gamma\inventory_i]
% 			\cup \batch_{i,j+1}[\gamma\inventory_i]
% 			~~~~
% 			\text{for all $j\in[2:\cnt_{i,T}-1]$}
% 			\end{align*}
% 			where $\batch_{i,j}[\gamma\inventory_i]$
% 			is the set of the first
% 			$\gamma\inventory_i$ units 
% 			added into $\batch_{i,j}$.
% 			By construction, 
% 			$\cup_{j=1}^{\cnt_{i, T}-1}
% 			\batchTilde_{i,j}$ contains 
% 			all $\finalinventoryi$ units 
% 			of product $i$.
% 			We also define $\batchidTilde$
% 			such that
% 			$k\in
% 			\batchTilde_{i,\batchidTilde}$.
% 			Note that for any product $i$
% 			and unit $k$,
% 			$\batchidTilde_{i,k}
% 			<\cnt_{i,\addtime(i,k)}$ 
% 			by construction.
% 			Recall  $\inventoryratio_{i,j,t} = 
%     \frac{\curinventory_{i, j, t}}
%     {|\batch_{i, j}|}
%     \cdot \indicator{j < \cnt_{i,t}}$.
% 			and thus 
% 			$
% 			\inventoryratio_{i,\batchidTilde,t}=
% 			\frac{\curinventory_{i,\batchidTilde,t}}
% 			{|\batch_{i,\batchidTilde}|} 
% 			\cdot \indicator{j < \cnt_{i,t}}
% 			=
% 			\frac{\curinventory_{i,\batchidTilde,t}}
% 			{|\batch_{i,\batchidTilde}|} 
% 			$
% 			for all time $t \geq \addtime(i,k)$.
% ////////////////
% 			
% 			we divide all units $k\in [\finalinventoryi]$
% 			such that $\addtime(i,k) \leq t$
% 			into three cases (with different dual assignment 
% 			constructions): 
% 			(i) unit $k$ with $\batchid=1$, which 
% 			satisfies $\addtime(i,k) = 1$ by construction;
% 			(ii) unit $k$ with $\batchid > 1$
% 			which is one of the first $\gamma \inventory_i$
% 			units added into $\batch_{i, \batchid}$;
% 			and 
% 			(iii) unit $k$ with $\batchid> 1$
% 			which is not one of the first $\gamma \inventory_i$
% 			units added into $\batch_{i, \batchid}$,
% 			and thus $\batchid = \cnt_{i, \addtime(i,k)} - 1
% 			< \cnt_{i, \addtime(i,k)}$
% 			by construction.
% 			The assignments of $\{\inventoryduali\}$
% 			in dual is constructed as follows:
% 			\begin{align*}
% 			\inventoryduali &= 
% 			\reward_i\left(
% 			\pen\left(
% 		\frac{\curinventory_{i, \batchidTilde, t}}
%     {|\batch_{i, \batchidTilde}|}
% 			\right) -
% 			\pen\left(
% \frac{\curinventory_{i, \batchidTilde, t}-1}
%     {|\batch_{i, \batchidTilde}|}
% 			\right)
% 			\right) 
% 			\\
% 			&
% 			~~~~~~~~~~~~
% 			~~~~~~
% 			\cdot
% 			\indicator{\text{a unit of product $i$ 
% 			from $\batch_{i,\batchidTilde}$
% 			is selected at time $t$}}~.
% % 			\\
% % 			\inventoryduali &= \reward_i\left(
% % 			\pen\left(\frac{\curinventory_{i,\batchid-1,t}}
% % 			{|\batch_{i,\batchid-1}|}
% % 			\right) -
% % 			\pen\left(\frac{\curinventory_{i,\batchid-1,t}
% % 			- 1}
% % 			{|\batch_{i,\batchid-1}|}
% % 			\right)
% % 			\right) 
% % 			~~~~~~
% % 			\text{$k$ in case (ii)}
% % 			\\
% % 			&
% % 			~~~~~~~~~~~~
% % 			~~~~~~
% % 			\cdot
% % 			\indicator{\text{a unit of product $i$ 
% % 			from $\batch_{i,\batchid-1}$
% % 			is selected at time $t$}}
% 	\end{align*}
	Note that for any product $i$ and unit $k$,
	by construction we have
	$\batchidTilde \leq 
	\cnt_{i, \addtimeTilde(i,k)} - 1$,
	i.e., 
	bin $\batch_{i}^{\batchidTilde}$
	is created no later 
	than time $\addtimeTilde(i,k)$.
	Thus, 
	$\curinventory_{i,t}^{\batchidTilde}$ 
	and $\inventorydual_{i,k,t}$
	are well-defined 
	for any time $t\geq \addtimeTilde(i,k)$.
	
	In the rest of analysis, we show the above randomized primal-dual assignments satisfy the conditions of \Cref{lem:random primal-dual} for 
		$\Gamma =
		\min\left\{
		\frac{e-1}{(2+\gamma)e 
		- e^{1-1/\mininventory}},
		\frac{e-1}{2e-
		e^{1-1/(\gamma\mininventory)}
		}
		\right\}$,
		which finishes the proof.
	\vspace{1mm}

	\noindent\emph{\rom{1}. Primal feasibility and dual feasibility in expectation.}
 The primal assignment is feasible, as EBIB (and in general any member of the BIB family) only offers inventory feasible assortments. 
 To show dual feasibility in expectation, 
 first note that $\pen(\cdot)$ is non-negative and monotone non-decreasing. 
 Therefore $\probduali\geq 0$ for all $t\in[\totaltime]$, and $\inventoryduali\geq 0$ for all 
 $i\in[n],k\in[\finalinventoryi],t\in[\addtimeTilde(i,k):\totaltime]$. 
 Next, we show for every $t\in[\totaltime]$ and
 $\indexnew\in\indexsetTilde(t)$, 
 the dual assignment satisfies the dual constraints corresponding to $\curalloc$ in expectation. 
 %Let $\indicator{\duration_{i, \tpre} \geq t - \tpre}$ be the indicator of the event that rental time of product $i$ at time $\tpre$ is at least 
	%$t - \tpre$. 
	For every product $i$ and unit $k$, 
	the following inequality holds at every time 
	$t\in[\addtimeTilde(i,k):\totaltime]$: 
	\begin{align}
		\label{eq:dual feasible ex post}
		\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-\duration_i + 1, \addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre} 
		\geq \reward_i
	\end{align}
	To see why 
	inequality~\eqref{eq:dual feasible ex post} holds, 
	consider on-hand units and  
	units not returned (from endogenous shock) of product $i$ 
	in bin $\batch_{i}^{\batchidTilde}$
	at time $t$. 
	Since the inventory level of bin
	$\batch_{i}^{\batchidTilde}$
	at time $t$ is 
	$\curinventory_{i,t}^{\batchidTilde}$, 
	there are $m \triangleq
	|\batch_{i}^{\batchidTilde}| 
	-
	\curinventory_{i,t}^{\batchidTilde}$ 
	units of product $i$ from this bin
	that are not returned at that moment. 
	Suppose these units were purchased at times
	$\tpre_1\leq\tpre_2\leq
	\dots\leq\tpre_{m}$,
	where $\max\{t-\duration_i + 1, \addtimeTilde(i,k)\}
	\leq \tpre_\ell \leq t - 1$
% 	and 
% 	$\indicator{\text{a unit of product $i$ 
% 			from $\batch_{i,\batchidTilde}$
% 			is selected at time $\tpre_\ell$}}=1$
	for all $\ell\in[m]$.
% 	\YF{This is the part why we need to introduce 
% 	$\EARPrime$, since those 
% 	$m$ units are allocated between
% 	$[\max\{t-\duration_i + 1, \addtimeTilde(i,k)\}, t - 1]$
% 	instead of 
% 	$[\max\{t-\duration_i + 1, \addtime(i,k)\}, t - 1]$,
% 	i.e., we need to have 
% 	dual variable $\theta_{i, k, t'}$
% 	for $t' \in [\addtimeTilde(i, k), \addtime(i,k)]$.}
	Additionally, the inventory level at time $\tpre_\ell$ is at most 
	$|\batch_{i}^{\batchidTilde}|
	- \ell + 1$,
	or equivalently we have
	$\curinventory_{i,\tpre_\ell}^{ \batchidTilde} 
	\leq  
	|\batch_{i}^{\batchidTilde}|
	-
	\ell + 1$ for all $\ell \in [m]$. This is true because at time $\tpre_\ell$ at least $\ell-1$ units of the product are not returned due to purchase happening at $\tpre_1,\ldots,\tpre_{\ell-1}$.
Because the penalty function $\pen(\cdot)$ is concave, we have:
	\begin{align}
	\begin{split}
	\label{eq:concave}
		\theta_{i, k, \tpre_\ell} &= 
		\reward_i\left(
		\pen\left(
		\frac{
		\curinventory_{i,
		\tpre_\ell}^{\batchidTilde}
		}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		-
	\pen\left(
		\frac{
		\curinventory_{i,
		\tpre_\ell}^{\batchidTilde} - 1
		}
		{|\batch_{i}^{\batchidTilde}|}
	\right)
	\right) 
	\geq
		\reward_i\left(
		\pen\left(
		\frac{|\batch_{i}^{\batchidTilde}| 
		- \ell + 1}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		-
	\pen\left(
	\frac{
	|\batch_{i}^{\batchidTilde}| - \ell}
	{|\batch_{i}^{\batchidTilde}|}\right)
	\right)
	\end{split}
	\end{align}
By applying \eqref{eq:concave},  we can prove inequality~\eqref{eq:dual feasible ex post}:
\begin{align*}
&\quad~
\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde,}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-\duration_i + 1, \addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre} 
		% \\
		% & 
		\geq
		\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+ 
		\displaystyle\sum\nolimits_{\ell = 1}^{m} 	\reward_i\left(
		\pen\left(
		\frac{
		\curinventory_{i,
		\tpre_\ell}^{\batchidTilde}
		}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		-
	\pen\left(
		\frac{
		\curinventory_{i,
		\tpre_\ell}^{\batchidTilde} - 1
		}
		{|\batch_{i}^{\batchidTilde}|}
	\right)
	\right) 
	\\
		&\geq
			\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+
		\displaystyle\sum\nolimits_{\ell = 1}^{m}\reward_i\left(
		\pen\left(
		\frac{|\batch_{i}^{\batchidTilde}| 
		- \ell + 1}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		-
	\pen\left(
	\frac{
	|\batch_{i}^{\batchidTilde}| - \ell}
	{|\batch_{i}^{\batchidTilde}|}\right)
	\right)
	\\
	&=
	\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+
	\displaystyle\sum\nolimits_{I = \curinventory_{i, t}^{\batchidTilde}}^{
	|\batch_{i}^{\batchidTilde}| - 1
	} 
		\reward_i\left(
			\pen\left(\frac{I + 1}{|\batch_{i}^{ \batchidTilde}|}\right) 
			-
			\pen\left(\frac{I}{|\batch_{i}^{ \batchidTilde}|}\right) 
		\right)=\reward_i\pen(1)=\reward_i
\end{align*}	

Now, for each time $t\in[\totaltime]$ 
and 
unit-specified assortment 
$\indexnew\in\indexsetTilde(t)$, consider this expression:
	\begin{align}
		\label{eq:dual LHS}
	\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}
	\end{align}
On the one hand, note that by taking expectation from \eqref{eq:dual LHS} we have 
\begin{equation}
\begin{split}
\label{eq:first-compare}
&\expect{
	\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}
		}\\
		=&\expect{\probduali} + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)
		\expect{\theta_{i,k,\tpre}} ~,
		\end{split}
\end{equation}
simply because of linearity of expectation. 
On the other hand, by taking expectation 
from $\probduali$
% \eqref{eq:dual LHS} 
by first conditioning on (i) history up to time $t$ (which includes inventory levels $\curinventory_{i,t}^{j}$ for each product $i$, bin $j$), 
and 
(ii) unit-specified assortment $\indexnew_t$ 
offered at time $t$, we have
\begin{align*}
% \label{eq:lambda conditional lowerbound} 
\begin{split}
\expect{
		\probduali  \condition\mathcal{F}_{t-1},\indexnew_t
		}
		&=
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew_t}
		\reward_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)
		\overset{(a)}{=}
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew_t}
		\reward_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\inventoryratio_{i, t}^{\batchid}
		\right)
		\end{split}
\end{align*}
where $\mathcal{F}_{t-1}$ 
denotes the history up to time $t$,
and 
inequality~(a) holds since 
for all $(i,k) \in \indexnew_t$ 
we have $\batchid< \cnt_{i,t}$ and thus
$\inventoryratio_{i,t}^{\batchid} = 
\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\cdot 
		\indicator{\batchid<\cnt_{i,t}}
		=\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}$.
Moreover, note that 
\begin{align*}
    &\sum_{(i,k)\in 
		\indexnew}
		\reward_i\choice_{t}(\indexnew, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
  % \\
  \overset{(a)}{=}
  \sum_{(i,k)\in 
		\indexnew}
		\reward_i\choice_{t}(\indexnew , i)
		\pen\left(
		\inventoryratio_{i, t}^{\batchidTilde}
		\right)
  % \\
  \leq 
  \max_{\indexnew^*\in \indexsetTilde(t)}~
    \sum_{(i,k)\in\indexnew^*} \reward_i \choice_t(\indexnew^*,i)
    \pen\left(
    \inventoryratio_{i, t}^{\batchidTilde}\right)
    \\
    \overset{(b)}{=} &
    \max_{\indexnew^*\in \indexsetTilde(t)}~
    \sum_{(i,k)\in\indexnew^*} \reward_i \choice_t(\indexnew^*,i)
    \pen\left(
    \max_{j^*\in [\cnt_{i, t} - 1]}
    \inventoryratio_{i, t}^{j^*}\right)
    % \\
    \overset{(c)}{=}
    % &
    \max_{\indexnew^*\in \indexset(t)}~
    \sum_{(i,k)\in\indexnew^*} \reward_i \choice_t(\indexnew^*,i)
    \pen\left(
    \max_{j^*\in [\cnt_{i, t} - 1]}
    \inventoryratio_{i, t}^{j^*}\right)
    \\
    \overset{(d)}{=} &
    \max_{\indexnew^*\in \indexset(t)}~
    \sum_{(i,k)\in\indexnew^*} \reward_i \choice_t(\indexnew^*,i)
    \pen\left(
    \inventoryratio_{i, t}^{\batchid}\right)
    % \\
    \overset{(e)}{=}
    % &
    \sum_{(i,k)\in\indexnew_t} \reward_i \choice_t(\indexnew_t,i)
    \pen\left(
    \inventoryratio_{i, t}^{\batchid}\right)
    % \\
    \overset{(f)}{=} ~
    \expect{
		\probduali  \condition\mathcal{F}_{t-1},\indexnew_t
		}
\end{align*}
We explain each step in this derivation:
For all $(i, k)\in \indexnew$, $\batchidTilde < \cnt_{i,t}$ due to the definition of $\batchidTilde$, which ensures 
equality~(a).
Since $\batchidTilde\in [\cnt_{i,t} - 1]$
by definition and choice function $\choice_t$ 
is independent of which unit is selected for every product,
equality~(b) holds.
Since set $\indexset(t)$ covers all
units in 
bins $[\cnt_{i, t} - 1]$
for each product $i$,
taking the maximum of $\indexnew$ over $\indexsetTilde(t)$
is equivalent to taking the maximum of $\indexnew$
over $\indexset(t)$,
which guarantees equality~(c).
Similar to equality~(b),
since choice function $\choice_t$ is independent of which unit is selected for every product,
equality~(d) holds.
Finally, equality~(e) holds because of the definition 
of $\indexnew_t$, and equality~(f) is what we shown above.

% 	and inequality~(d) holds due to construction 
% 	of $\indexnew'$.
	Now consider
	the expectation of 
	\eqref{eq:dual LHS} 
	by conditioning on 
	$\mathcal{F}_{t-1},\indexnew_t$,
	\begin{align*}
		&\expect{
		\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre} \condition\mathcal{F}_{t-1},\indexnew_t
		}\nonumber\\
		&~~\overset{(a)}{\geq}
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew}
		\reward_i\choice_{t}(\indexnew, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		+	
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew}
		\displaystyle\sum\nolimits_{\tpre =
		\max\{t-\duration_i+1,\addtimeTilde(i,k)\}}^{t - 1}
		\choice_t(\indexnew,i) 
		\inventorydual_{i,k, \tpre} \nonumber \\
		&~~=
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew} 
		\choice_{t}(\indexnew,i)
		\left(\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
		{|\batch_{i}^{\batchidTilde}|}
		\right)+ \displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,\addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre}  \right)
		\nonumber  \overset{(b)}{\geq} \displaystyle\sum\nolimits_{(i,k)\in\indexnew} 
		\reward_i\choice_t(\indexnew,i)~,\nonumber
	\end{align*}
where
inequality~(a) holds by  
applying the inequality of the conditional expectation of $\probduali$ above
and dropping non-negative terms related to 
$\inventorydual_{i,k,t}$ for all $(i,k)\in \indexnew$;
and 
inequality~(b) holds because of  inequality~\eqref{eq:dual feasible ex post}. Therefore, by taking another expectation over $\indexnew_t$ and  $\mathcal{F}_{t-1}$, we have:
\begin{equation}
\label{eq:second-compare}
\expect{
\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}
		}\geq \displaystyle\sum\nolimits_{i = 1}^n 
		\reward_i\choice_t(\indexnew,i)
\end{equation}
Combining \eqref{eq:first-compare} and \eqref{eq:second-compare} shows  feasibility in expectation of the dual assignment.
%	\begin{align}
%		\label{eq:dual feasible ex post final}
%		\eqref{eq:feasibility ex post} 
%		\geq 
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice
%		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
%		&+	
%		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
%		\indicator{\duration_{i, \tpre} \geq t - \tpre}
%		\curchoice \theta_{i, \tpre}  
%	\end{align}
%	Applying inequality \eqref{eq:dual feasible ex post}, it implies
%	\begin{align*}
%		\eqref{eq:feasibility ex post} 
%		\geq 
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice.
%	\end{align*}
%	where $
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice$
%		is the right hand side of the dual constraint corresponding to the
%		primal variable $\curalloc$.
%	Having this inequality,
	
	\vspace{1mm}
	
	\noindent\emph{\rom{2}. Comparing objective values of primal and dual.} 
	We consider the value increments 
	in both primal 
	and dual for each time period separately. 
	Given history up to time $t$ 
	and offering unit-specified assortment 
	$\indexnew_t$ at time $t$, the conditional expected increments (over randomness of the choice of consumer $t$) in primal and dual are
	\begin{align*}
		&\expect{
		\Delta(\text{Primal})
		\condition
		\mathcal{F}_{t-1},\indexnew_t}= \displaystyle\sum\nolimits_{(i,k)\in \indexnew_t} 
		r_i\choice_{t}(\indexnew_t, i) \\
		&\expect{\Delta(\text{Dual})
		\condition
		\mathcal{F}_{t-1},
		\indexnew_t} 
		=
		\displaystyle\sum\nolimits_{i\in[n]}
		\displaystyle\sum\nolimits_{k\in [\finalinventoryi]:
		\addtimeTilde(i,k)\leq t}
		\expect{\inventorydual_{i,k,t}
		\condition 
		\mathcal{F}_{t-1},\indexnew_t
		}
		+
		\expect{\probdual_{t}
		\condition
		\mathcal{F}_{t-1},\indexnew_t}
		\\
		\overset{(a)}=&
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		\displaystyle\sum\nolimits_{k'\in\batchTilde_{i}^{\batchid}}
		\expect{\inventorydual_{i,k',t}
		\condition 
		\mathcal{F}_{t-1},\indexnew_t
		}
		+
		\expect{\probdual_{t}
		\condition
		\mathcal{F}_{t-1},\indexnew_t}
		\\
		=&
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		\displaystyle\sum\nolimits_{k'\in
		\batchTilde_{i}^{\batchid}}
		\reward_i
		\choice_{t}(\indexnew_t, i)
		\left(
			\pen\left(
			\frac{\curinventory_{i,t}^{\batchidTildePrime}}
		{|\batch_{i}^{\batchidTildePrime}|}
			\right)
			-
			\pen\left(
			\frac{
			\curinventory_{i,t}^{\batchidTildePrime}-1
			}
		{|\batch_{i}^{\batchidTildePrime}|}
			\right)
		\right)
		% \\
		% &~~~~~~~~~
		% \qquad 
  +
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		r_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)\\
		\overset{(b)}=&
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		\displaystyle\sum\nolimits_{k'\in
		\batchTilde_{i}^{\batchid}}
		\reward_i
		\choice_{t}(\indexnew_t, i)
		\left(
			\pen\left(
			\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
			\right)
			-
			\pen\left(
			\frac{
			\curinventory_{i,t}^{\batchid}-1
			}
		{|\batch_{i}^{\batchid}|}
			\right)
		\right)
		% \\
		% &~~~~~~~~~
		% \qquad
  +
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		r_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)\\
		=&
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		|\batchTilde_{i}^{\batchid}|
		\reward_i
		\choice_{t}(\indexnew_t, i)
		\left(
			\pen\left(
			\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
			\right)
			-
			\pen\left(
			\frac{
			\curinventory_{i,t}^{\batchid}-1
			}
		{|\batch_{i}^{\batchid}|}
			\right)
		\right)
		% \\
		% &~~~~~~~~~
		% \qquad
  +
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		r_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)
	\end{align*}
	where equality~(a) holds since 
	$\expect{\inventorydual_{i,k',t}\condition\mathcal{F}_{t-1},\indexnew_t} = 0$
	for all other units;
% 	equality~(b) is by the construction of 
% 	$\inventorydual_{i,j,k'}$;
	and 
	equality~(b) holds since $\batchidTildePrime=\batchid$
	for all $k' \in \batchTilde_{i}^{\batchid}$ by definition. Thus, to show $\expect{\Delta\textrm{(Primal)}}\geq \Gamma \cdot\expect{\Delta\textrm{(Dual)}}$--- which in turn shows $\expect{\textrm{obj(Primal)}}\geq \Gamma \cdot\expect{\textrm{obj(Dual)}}$---it is sufficient to show
	\begin{align}
		\label{eq:increament}
	|\batchTilde_{i}^{\batchid}|
		\left(
			\pen\left(	\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
			\right)
			-
			\pen\left(
	\frac{\curinventory_{i,t}^{\batchid}-1}
		{|\batch_{i}^{\batchid}|}
			\right)
		\right)
		+
		\pen\left(
			\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
	\right)
		\leq \tfrac{1}{\Gamma}
	\end{align}
The exponential penalty function $\exponential$ satisfies the following differential equation:
	\begin{align}
	\label{eq:exponential differential equation}
	    \pen'(x) +\pen(x)= \frac{e}{e-1}
	\end{align}
Therefore, we have 
	\begin{align}
	\label{eq:increament 2}
	\begin{split}
		\textrm{LHS of}~\eqref{eq:increament}  &\overset{(a)}{\leq} 
		\pen\left(
			\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right) 
		+
			\frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
			\cdot
		\pen'\left(
		\frac{\curinventory_{i,t}^{\batchid}-1}
		{|\batch_{i}^{\batchid}|}
		\right)  
  % \\
		% &
  \overset{(b)}{=} 
			\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)  
		+
			\frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
			\cdot
		\left(\frac{e}{e - 1} 
			-
		\pen\left(
			\frac{\curinventory_{i,t}^{\batchid}-1}
		{|\batch_{i}^{\batchid}|}
		\right) 
		\right)
	\end{split}
		\end{align}
		where~(a) holds due to concavity of $\pen$, and~(b) holds due
		to \eqref{eq:exponential differential equation}.
		Now we discuss two cases
		$\batchid = 1$
and $\batchid \geq 2$ separately.
For $\batchid= 1$,
by construction, $|\batch_{i}^{1}|\geq \inventory_i$
and $0\leq |\batchTilde_{i}^{1}| - |\batch_{i}^{1}| \leq
\gamma\inventory_i$. Thus,
		\begin{align*}
		    \textrm{RHS of}~\eqref{eq:increament 2}
		    &\leq
		    \frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
			% \cdot
		\frac{e}{e - 1} 
		+
			\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)  
		-
			\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}-1}
		{|\batch_{i}^{\batchid}|}
		\right)  
		\leq 
		 \frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
			% \cdot
		\frac{e}{e - 1} 
		+
		\pen\left(\frac{1}{|\batch_{i}^{\batchid}|}\right)
		-
		\pen\left(\frac{0}{|\batch_{i}^{\batchid}|}\right)
		\\
		&\leq
		\left(1+\gamma\right)\frac{e}{e-1}
		+
		\frac{e-e^{1-1/\inventory_i}}{e-1}
		\leq 
		\left(1+\gamma\right)\frac{e}{e-1}
		+
		\frac{e-e^{1-1/\mininventory}}{e-1}
		\leq \frac{1}{\Gamma}
		\end{align*}
For $\batchid \geq 2$,
by construction,
$|\batch_{i}^{\batchid}|\geq \gamma\inventory_i$
and 
$|\batchTilde_{i}^{\batchid}|
\leq |\batch_{i}^{\batchid}|$.
Thus,
		\begin{align*}
		    \textrm{RHS of}~\eqref{eq:increament 2}
		    &=
		    \frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
			\cdot
		\left(\frac{e}{e - 1} 
		+
			\pen\left(
		\frac{\curinventory_{i}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)  
		-
			\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}-1}
		{|\batch_{i}^{\batchid}|}
		\right) 
		\right)
		% \\
		% &
		+
		    \left(1-\frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
		    \right)
			\pen\left(
		\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\right)  
		\\
		&\leq 
		 \frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
			\cdot
		\left(\frac{e}{e - 1} 
		+
		\frac{e-e^{1-1/(\gamma\inventory_i)}}{e-1}
		\right)
		+
		1-
		\frac{|\batchTilde_{i}^{\batchid}|}
			{|\batch_{i}^{\batchid}|}
		\\
		&\leq
		\frac{e}{e-1}
		+
		\frac{e-e^{1-1/(\gamma\inventory_i)}}{e-1}
		\leq 
	\frac{e}{e-1}
		+
		\frac{e-e^{1-1/(\gamma\mininventory)}}{e-1}
		\leq \frac{1}{\Gamma}
		\end{align*}
Combining two cases,
invoking \Cref{lem:tilde relaxation} and \Cref{lem:random primal-dual}, and letting $\mininventory$ approach infinity finishes the proof.
\end{proof}
\end{comment}

==> Paper/IBB-proof.tex <==
\label{sec:IBB proof}
\label{sec:IAP}
In this section,
we prove 
\Cref{thm:concave competitive ratio} for 
general concave penalty functions. Recall the two challenges mentioned at the beginning of \Cref{sec:EIBB}.
In the proof of 
\Cref{thm:exponential competitive ratio} for EIBB,
we address Challenge~(i) by considering unit-specified
dual assignments using the bins.
This proof also overcomes Challenge~(ii),
since we have 
the differential 
equation~\eqref{eq:exponential differential equation} 
(i.e., $\pen'(x)+\pen(x) = e/(e-1)$ for all $x\in[0,1]$)
for exponential penalty function,
and thus we are able to argue 
the value increment in both primal and dual
is bounded by $1-\sfrac{1}{e}$ per period.


For general concave penalty functions beyond exponential, i.e., functions that do not satisfy $\pen'(x)+\pen(x) = c$ for a given constant $c$ for all $x\in[0,1]$, the previous argument in the proof of \Cref{thm:exponential competitive ratio} fails to hold. 
One idea to is then to compare the value of primal and dual 
for all time periods together through an argument similar to \cite{GNR-14} when there is no inventory shock, and extend the proof of  \Cref{thm:exponential competitive ratio} to general penalty functions accordingly. Importantly, this last argument in \cite{GNR-14} requires inventory levels to be weakly decreasing over time, which is a critical property that is missing in our problem by default. 

\subsection{A Combinatorial Problem to Rescue}
\label{sec:IAP-def}
To avoid the issue due to the non-monotonicity of inventory levels, we follow a similar randomized primal-dual argument 
as in \Cref{thm:exponential competitive ratio} 
but with a more involved 
algorithmically constructed dual solution.
Specifically, we introduce a sub-problem termed as \emph{Interval Assignment Problem (IAP)},
and an algorithm to solve it. We this algorithm as a guide 
to construct the dual solution. 



\noindent\textbf{How does IAP help with obtaining the desired competitive ratio?} Before we show the algorithmic construction of
a feasible solution to IAP, we highlight 
how we use it in the dual assignment construction.
Recall that in the proof of \Cref{thm:exponential competitive ratio},
we define dual variables $\{\probdual_t,\inventorydual_{i,k,t}\}$.
For each product $i$ and bin $j$,
consider the following 
instance of the Interval Assignment Problem (IAP)
in \Cref{def:IAP}
separately.
Let 
%it has been allocated at time 
$\texttt{alloc}_{i}^{j} = \{t_1, t_2, \dots, t_s\}$
be the time periods when a unit of product $i$ from 
$\batch_{i}^{ j}$ 
is selected.
Consider the instance of IAP with $s$ intervals
$\{[t_1, t_1 + \duration_i], \dots, 
[t_s, t_s + \duration_i]\}$.
Let 
$\{\assign_{i,t}^{j}\}_{t\in \texttt{alloc}_{i}^{j}}$ 
be the assignment solved in IAP
% with 
% decreasing concave $\bar\pen(x) \triangleq 
% \pen(|\batch_{i}^{j}| - x)$
for bin $j$ of product $i$
and let 
$\pseudoinventory_{i, t}^{j} = 
|\batch_{i}^{j}| - \assign_{i,t}^{j}$ 
if $t \in \texttt{alloc}_{i}^{j}$
and $\pseudoinventory_{i,t}^{j} = 1$ otherwise.
    Consider the following assignments of 
    dual variables:
	\begin{align*}
\probduali &= 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		\reward_i 
		\pen\left(
		\frac{\curinventory_{i, t}^{\batchid}}
    {|\batch_{i}^{\batchid}|}
		\right)
		\cdot
			\indicator{\text{a unit from $\batch_{i}^{\batchid}$ is selected at time $t$}} \\
			\inventoryduali &= 
			\reward_i\left(
			\pen\left(
		\frac{\pseudoinventory_{i, t}^{\batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
			\right) -
			\pen\left(
\frac{\pseudoinventory_{i, t}^{\batchidTilde}-1}
    {|\batch_{i}^{\batchidTilde}|}
			\right)
			\right) 
% 			\\
% 			&
% 			~~~~~~~~~~~~
% 			~~~~~~
			\cdot
			\indicator{\text{a unit  
			from $\batch_{i}^{\batchidTilde}$
			is selected at time $t$}}~.
	\end{align*}
This dual construction is similar to 
the construction in \Cref{thm:exponential competitive ratio} for EIBB. 
The only difference is that we replace 
$\curinventory_{i,t}^{\batchidTilde}$
with 
$\pseudoinventory_{i,t}^{\batchidTilde}$ 
in $\{\inventorydual_{i,k,t}\}$. 
Next we briefly discuss the usage of
three properties in IAP solution. 
\emph{Local Dominance} is invoked 
in the argument of dual feasibility to show
	\begin{align*}
		\reward_i
		\pen\left(
		\frac{\curinventory_{i, t}^{\batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-\duration_i + 1, \addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre} 
		\geq \reward_i
	\end{align*}
Both \emph{Global Dominance}
and \emph{Partition Monotonicity}
are used in the comparison 
of objective values in primal and dual.
In particular, by \emph{Global Dominance}
we can replace the total contribution 
of $\{\probduali\}$ as a function 
of $\{\curinventory_{i,t}^{j}\}$
with a function of $\{\pseudoinventory_{i,t}^{j}\}$.
Invoking \emph{Partition Monotonicity},
for every subgroup defined in this property,
$\{\pseudoinventory_{i,t}^{j}\}$ is monotone decreasing,
and thus enables us to use a modified version of the argument 
used in the proof of \Cref{thm:exponential competitive ratio} to finish the proof of our main theorem.

We show the existence of a feasible solution for IAP in \Cref{sec:alg-IAP}. In particular, we present an auxiliary algorithm to generate the solution. 

\subsection{Algorithmic Solution for IAP}
\label{sec:alg-IAP}
To show the existence of a feasible solution for IAP,
we present \Cref{alg:interval assignment} and show its correctness.


\begin{algorithm}[htb]
 	\caption{Interval Assignment Solver
}\label{alg:interval assignment}
 	\KwIn{$s$ intervals $\{[a_1, b_1], \dots, [a_s, b_s]\}$}
 	\vspace{2mm}
 	
Initialize an assignment vector
$\assign_i \gets 0$ for all $i \in [s]$.


Initialize a pointer vector 
$\pfather_i \gets -1$ for all $i \in [s]$. 


Initialize a pointer vector
$\pmother_i \gets -1$  for all $i \in [s]$.


Initialize the remaining interval set 
$\remaining \gets \{1, 2, \dots, s\}$.



\tcc{define $\remainingcontain_i = \contain_i \cap \remaining$}
% and $\remainingcontainni = |\remainingcontain_i|$}


 	\While{$\remaining$ is not empty}{
 	
Find the interval $i$ with the largest index 
in the remaining interval set $\remaining$
where $\remainingcontainni$ is maximized, 
i.e., $i \gets\,
\argmax_{i\in \remaining} \{\remainingcontainni
\}$. 



Find the interval $j$ with the smallest index %left most starting point
in the remaining interval set $\remaining$
which
covers position $a_i$,
i.e., $j \gets \min \remainingcontain_i$.



Set $\assign_j \gets \remainingcontainni$ and $\pmother_j \gets i$.



\For{all $k \in [s] / \remaining$ such that 
$j \in \contain_{\pmother_k}$ and $\assign_k = \assign_j + 1$}{
Set $\pfather_k \gets j$. 
}
Remove interval $j$ from the remaining interval set $\remaining$ %, and update $C(t)$ 
%for all remaining interval $t$,\par
%\hskip\algorithmicindent  
i.e., set
$\remaining \gets \remaining / \{j\}$.
%$C(t) = \{\tpre \in R \given 
%\tpre \leq t, f(\tpre) \geq t\}$.
%\end{varwidth}

}
\textbf{return} $\{\assign_1, \dots, \assign_s\}$.
\end{algorithm}

\begin{algorithm}[htb]
 	\caption{Partition Construction
}\label{alg:partition monotonicity construction}
 	\KwIn{$s$ intervals $\{[a_1, b_1], \dots, [a_s, b_s]\}$;
 	and $\{\assign_{i}, \pfather_i\}$
 	from \Cref{alg:interval assignment}}
 	\vspace{2mm}
 	
Initialize $\kappa \gets 0$.


Initialize the remaining interval set $\remaining\gets\{1,2,\dots, s\}$.


\While{$\remaining$ is not empty}{
 	

Find the interval $i\in \remaining$
such that $i\not= \pfather_j$ for all $j\in [s]$. 



$\kappa \gets \kappa+1$



Create $A^{\kappa} \gets \{i\}$.



\While{$\pfather_i \not=  -1$}{


$i\gets \pfather_i$.


$A^{\kappa} \gets A^{\kappa} \cup \{i\}$.
}
}
\textbf{return} $\{A_1, \dots, A_\kappa\}$.
\end{algorithm}



\begin{proof}
In each iteration, \Cref{alg:interval assignment} 
pins down the assignment for a remaining interval and then remove it.
Thus, the algorithm terminates and outputs an assignment $\{\assign_1, \dots, \assign_s\}$.
We next show this assignment satisfies \emph{Local Dominance}, \emph{Global Dominance}
and \emph{Partition Monotonicity}.

\noindent\emph{\rom{1}. Local Dominance.}
%\paragraph{Local Dominance} 
For each interval $i \in [s]$,
consider $j_1, j_2, \dots \in \contain_i$ in the order which they are
removed from the algorithm:
for the $k$-th removed interval $j_k \in \contain_i$,
at that time $\remainingcontainni$ is $\containni - k + 1$,
which guarantees that $\assign_{j_k}$ is at least $\containni - k + 1$.
Thus, \emph{Local Dominance} is satisfied.


\noindent\emph{\rom{2}. Global Dominance.}
%\paragraph{Global Dominance}
We prove this by induction. Consider the reverse order of intervals removed
from the remaining interval set $\remaining$ in the algorithm,
i.e., we set $\remaining = \emptyset$ as the base case and then add intervals back to $\remaining$
in the reverse order which they have been removed in the algorithm. 
Our induction hypothesis is that restricting to intervals in $\remaining$ the
\emph{Global Dominance} holds,
i.e., for any decreasing and concave function $\bar\pen$,
\begin{align}
\label{eq:global dominance}
\sum_{i\in \remaining} \bar\pen(\assign_i) \geq \sum_{i \in \remaining} \bar\pen(\remainingcontainni).
\end{align}

\emph{Base Case ($\remaining = \emptyset$):} In this case, the induction hypothesis holds trivially.

\emph{Inductive Step:}  Suppose the induction hypothesis holds before we add interval $i$ 
with $\assign_{i}$ back
to $\remaining$. 
Let $m = \assign_{i} - 1$.
To make it clear, let $\remaining$ to be the remaining interval set before we add interval $i$,
and $\remaining'$ to be the remaining interval set after we add interval $i$, i.e., 
$\remaining' = \remaining \cup\{i\}$.
%Let $\assign^{-1}(c) = |\{j \in W: \assign_j = c\}|$
%and 
%$\containn^{-1}(c) = |\{j \in W: |\contain_j \cap W| = c\}|$.
Next we consider the increment of both sides in 
\eqref{eq:global dominance}
after 
we add interval $i$ into $\remaining$.
The left hand side of \eqref{eq:global dominance} increases by $\bar\pen(m + 1)$.
%$\assign^{-1}(k)$ increases by one 
%while $\assign^{-1}(k')$ does not change for all $k' \not=k$.
For the right side, since $\assign_i = m + 1$,
there exist $m$ intervals $j_1, j_2, \dots j_m \in \remaining$
which 
%such that interval $j_k$ 
cover position $a_{\pmother_i}$,
and $i < j_k$ (otherwise, $j_k$ should be removed early than $i$ in the algorithm)
for all $k\in[m]$.
This implies that interval $i$ covers position $a_{j_k}$ 
for all $k \in[m]$.
Without loss of generality, we assume $j_1 < j_2 < \dots < j_m$,
then $
|\remainingcontain_{j_k}|\geq k$.
Hence, once we add interval $i$ into $W$,
the right hand side of \eqref{eq:global dominance}
increases by 
\begin{align*} 
\bar\pen(|\contain_i^{\remaining'}|) + 
\sum_{j\in \remaining}
\left(
\bar\pen(|\contain_{j}^{\remaining'}|) - 
\bar\pen(|\contain_{j}^{\remaining}|)
\right) 
&\leq \bar\pen(|\contain_i^{\remaining'}|) + 
\sum_{k\in[m]}
\left(
\bar\pen(|\contain_{j_k}^{\remaining'}|) - 
\bar\pen(|\remainingcontain_{j_k}|)
\right) \\
&=
\bar\pen(|\contain_i^{\remaining'}|) + 
\sum_{k\in[m]}
\left(\bar\pen(|\remainingcontain_{j_k}| + 1) - 
\bar\pen(|\remainingcontain_{j_k}|)\right) 
\\
&\overset{(a)}{\leq} 
\bar\pen(1) + 
\sum_{k \in [m]}
(
\bar\pen(k + 1) - \bar\pen(k)
)\\
&= \bar\pen(m + 1)
\end{align*}
where (a) holds because $\bar\pen$ is decreasing and concave.
Applying the induction hypothesis (before we add interval $i$),
the inductive claim (after we add interval $i$) holds,
which finishes the induction.

\noindent\emph{\rom{3}. Partition Monotonicity.}
%\paragraph{Partition Monotonicity}
We first introduce the following two claims:
(a) for each interval $i\in[s]$, there is at most one interval $j$ such that
$\pfather_j = i$;
(b) for each interval $i\in[s]$ with $\assign_i > 1$, $\pfather_i \not= -1$.  
Note that claim (a) and (b) together imply that $\{\pfather_1, \dots, \pfather_s\}$ 
defines a partition which satisfies \emph{Partition Monotonicity} 
from \Cref{alg:partition monotonicity construction}.

Next, we show claim (a) and claim (b) separately.
We show claim (a) by contradiction. 
Suppose there exists interval $i$, $j_1$ and $j_2$ such that 
$\pfather_{j_1} = \pfather_{j_2} = i$.
By the construction of the algorithm,
$\assign_{j_1} = \assign_{j_2} = \assign_i + 1$.
Now, consider case by case.

\vspace{1.5mm}

\noindent\textbullet\ \emph{Case 1 ($i < j_1$ or $i < j_2$):} Without loss of generality, we assume $i < j_1$,
and the case $i < j_2$ is symmetric.
%Consider the moment when the algorithm 
%removes interval $j_1$ due to $\pmother_{j_1}$.
By the construction of the algorithm,
$\pfather_{j_1} = i$ implies 
$i \in \contain_{\pmother_{j_1}}$. 
%interavl $i$ also covers position $a_{\pmother_{j_1}}$,
This leads to a contradiction, because 
if $i < j_1$, interval $i$ should be removed early than interval $j_1$ in the algorithm 
which implies $\assign_i \geq \assign_{j_1}$.

\noindent\textbullet\ 
\emph{Case2 ($j_1, j_2 < i$):}

\hspace{5mm}\noindent\textbullet\ 
\emph{Case 2a ($\pmother_{j_1} < \pmother_{j_2}$ or $\pmother_{j_2} < \pmother_{j_1}$):}
W.L.O.G., we assume $\pmother_{j_1} < \pmother_{j_2}$ ($\pmother_{j_2} < \pmother_{j_1}$ is similar):

\hspace{10mm}\noindent\textbullet\ \
\emph{Case 2a1 (interval $j_1$ is removed before interval $j_2$):}
In this case, consider the moment 
when the algorithm removes $j_1$ due to interval $\pmother_{j_1}$.
By the construction of the algorithm, since $j_1$ is removed before $j_2$,
it implies
$|\remainingcontain_{\pmother_{j_1}}| > |\remainingcontain_{\pmother_{j_2}}|$.
Thus,
$\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
contradiction.

\hspace{10mm}\noindent\textbullet\ \
\emph{Case 2a2 (interval $j_2$ is removed before interval $j_1$):}
In this case, consider the moment 
when the algorithm remove $j_2$ due to interval $\pmother_{j_2}$.
Notice that interval $j_2$ also covers position $a_{\pmother_{j_1}}$,
i.e., $j_2 \in \contain_{\pmother_{j_1}}$.
By the construction of the algorithm, since $j_2$ is removed before $j_1$,
it implies
$|\remainingcontain_{\pmother_{j_1}}|  \leq |\remainingcontain_{\pmother_{j_2}}|$.
Thus, once the algorithm removed $j_2$, 
$|\contain_{\pmother_{j_1}}^{\remaining/\{j_2\}}|$ (which is an upper bound
of $\assign_{j_1}$) 
becomes strictly smaller than 
$|\remainingcontain_{\pmother_{j_2}}|$ (which is equal to $\assign_{j_2}$), %which 
%implies $\assign_{j_1}$ is strictly smaller than $\assign_{j_2}$,
contradiction.


\hspace{5mm}\noindent\textbullet\ 
\emph{Case 2b ($\pmother_{j_1} = \pmother_{j_2}$):}
Without loss of generality, we assume interval $j_1$ is removed before interval $j_2$,
and the case where interval $j_2$ is removed before interval $j_1$ is 
symmetric.
Let $\pmother^* = \pmother_{j_1} = \pmother_{j_2}$. Consider the moment
when the algorithm removes $j_1$ due to $\pmother^*$.
By the construction of the algorithm,
$\assign_{j_1} = 
|\remainingcontain_{\pmother^*}|$
and $\assign_{j_2} \leq |\contain_{\pmother^*}^{\remaining/\{j_1\}}|
= |\remainingcontain_{\pmother^*}| - 1$.
Thus, $\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
which is a contradiction.

\vspace{1.5mm}

We show claim (b) as follows. For any interval $i$
with $\assign_i > 1$,
consider the next removed interval $j$ %which covers 
%position $a_{q_i}$ and is the first interval removed 
among
$\contain_{\pmother_i}$ after the algorithm removes interval $i$.
It is sufficient to show $\assign_j = \assign_i - 1$,
which implies that algorithm set $\pfather_i = j$ when it removes interval $j$.
Since $j$ is the next interval removed among $\contain_{\pmother_i}$ after 
interval $i$, $\assign_i - 1\leq \assign_j \leq \assign_i$.
To show $\assign_j < \assign_i$, we use contradiction.
Suppose $\assign_j = \assign_i$. If $i\in\contain_{\pmother_j}$,
this implies that at the moment when the algorithm removes $i$, 
$
\assign_i = |\contain_{\pmother_i}^{\remaining}|
\geq
|\contain_{\pmother_j}^{\remaining}| \geq \assign_j + 1 = \assign_i + 1
$, contradiction.
If $i \not\in \contain_{\pmother_j}$, since $i < j$, 
it implies that $\pmother_i < \pmother_j$ and
at the moment when the algorithm removes $i$,
$|\contain_{\pmother_i}^\remaining|
=
\assign_i
=\assign_j 
\leq |\contain_{\pmother_j}^\remaining|
$, contradiction.
% \qedhere
\end{proof}

==> Paper/alg-IAP-partition.tex <==

\begin{algorithm}[htb]
 	\caption{\textsc{Partition Construction}
}\label{alg:partition monotonicity construction}
\label{alg:IAP partition}
 	\KwIn{sequence of $s$ intervals $\{[a_1, b_1], \dots, [a_s, b_s]\}$;
 	and its $\{\assign_{i}, \pfather_i\}_{i\in[s]}$
 	from \Cref{alg:interval assignment}}
 	\KwOut{partition $A_1, \dots, A_\kappa$ of $[s]$}
 	
initialize $\kappa \gets 0$

initialize remaining interval set $\remaining\gets\{1,2,\dots, s\}$

\While{$\remaining$ is not empty}{

find interval $i\in \remaining$ such that $i\not= \pfather_j$ for all $j\in [s]$. 

update $\kappa \gets \kappa+1$

initialize $A_{\kappa} \gets \{i\}$

\While{$\pfather_i \not=  -1$}{
update $i\gets \pfather_i$

update $A_{\kappa} \gets A_{\kappa} \cup \{i\}$
}
}
\textbf{return} $\{A_1, \dots, A_\kappa\}$
\end{algorithm}

==> Paper/alg-IB.tex <==

\begin{algorithm}
 	\caption{\textsc{\IB}~(IB)}
 	\label{alg:IB}
 	\KwIn{penalty function $\pen$}
 	
 	\For{each time period $t\in[T]$}{ 
 	\tcc{consumer $t$ with choice model $\choice_t$ arrives.} 
 	
    \tcc{$\repleni$ new units of product $i$ are added due to exogenous shock.}
    
    \tcc{denote $\curinventory_{i,t}$ by the inventory level 
    of product $i$ at time period $t$.}
    

    solve $\assortment_t\gets
    \argmax\nolimits_{
    \assortment\in \assortmentspace}
    \sum_{i\in \assortment} 
    \reward_i
    \pen\left(\sfrac{\curinventory_{i, t}}
    {\inventory_i}
    \right)\cdot \choice_{t}(\assortment, i)$.
 	
 	allocate assortment $\assortment_t$ to consumer $t$.
 	}
\end{algorithm}

==> Paper/apx-IAP-alg.tex <==

\subsection{Algorithmic Solution for IAP}
\label{sec:alg-IAP}
To show the existence of a feasible solution for IAP,
we present \Cref{alg:interval assignment} and show its correctness.


\begin{algorithm}[htb]
 	\caption{Interval Assignment Solver
}\label{alg:interval assignment}
 	\KwIn{$s$ intervals $\{[a_1, b_1], \dots, [a_s, b_s]\}$}
 	\vspace{2mm}
 	
Initialize an assignment vector
$\assign_i \gets 0$ for all $i \in [s]$.


Initialize a pointer vector 
$\pfather_i \gets -1$ for all $i \in [s]$. 


Initialize a pointer vector
$\pmother_i \gets -1$  for all $i \in [s]$.


Initialize the remaining interval set 
$\remaining \gets \{1, 2, \dots, s\}$.



\tcc{define $\remainingcontain_i = \contain_i \cap \remaining$}
% and $\remainingcontainni = |\remainingcontain_i|$}


 	\While{$\remaining$ is not empty}{
 	
Find the interval $i$ with the largest index 
in the remaining interval set $\remaining$
where $\remainingcontainni$ is maximized, 
i.e., $i \gets\,
\argmax_{i\in \remaining} \{\remainingcontainni
\}$. 



Find the interval $j$ with the smallest index %left most starting point
in the remaining interval set $\remaining$
which
covers position $a_i$,
i.e., $j \gets \min \remainingcontain_i$.



Set $\assign_j \gets \remainingcontainni$ and $\pmother_j \gets i$.



\For{all $k \in [s] / \remaining$ such that 
$j \in \contain_{\pmother_k}$ and $\assign_k = \assign_j + 1$}{
Set $\pfather_k \gets j$. 
}
Remove interval $j$ from the remaining interval set $\remaining$ %, and update $C(t)$ 
%for all remaining interval $t$,\par
%\hskip\algorithmicindent  
i.e., set
$\remaining \gets \remaining / \{j\}$.
%$C(t) = \{\tpre \in R \given 
%\tpre \leq t, f(\tpre) \geq t\}$.
%\end{varwidth}

}
\textbf{return} $\{\assign_1, \dots, \assign_s\}$.
\end{algorithm}

\begin{algorithm}[htb]
 	\caption{Partition Construction
}\label{alg:partition monotonicity construction}
 	\KwIn{$s$ intervals $\{[a_1, b_1], \dots, [a_s, b_s]\}$;
 	and $\{\assign_{i}, \pfather_i\}$
 	from \Cref{alg:interval assignment}}
 	\vspace{2mm}
 	
Initialize $\kappa \gets 0$.


Initialize the remaining interval set $\remaining\gets\{1,2,\dots, s\}$.


\While{$\remaining$ is not empty}{
 	

Find the interval $i\in \remaining$
such that $i\not= \pfather_j$ for all $j\in [s]$. 



$\kappa \gets \kappa+1$



Create $A^{\kappa} \gets \{i\}$.



\While{$\pfather_i \not=  -1$}{


$i\gets \pfather_i$.


$A^{\kappa} \gets A^{\kappa} \cup \{i\}$.
}
}
\textbf{return} $\{A_1, \dots, A_\kappa\}$.
\end{algorithm}

\begin{lemma}
For any input instance,
the solution of Interval Assignment Problem exists. Specifically, 
\Cref{alg:interval assignment} outputs such a solution.
\end{lemma}

\begin{proof}
In each iteration, \Cref{alg:interval assignment} 
pins down the assignment for a remaining interval and then remove it.
Thus, the algorithm terminates and outputs an assignment $\{\assign_1, \dots, \assign_s\}$.
We next show this assignment satisfies \emph{Local Dominance}, \emph{Global Dominance}
and \emph{Partition Monotonicity}.

\noindent\emph{\rom{1}. Local Dominance.}
%\paragraph{Local Dominance} 
For each interval $i \in [s]$,
consider $j_1, j_2, \dots \in \contain_i$ in the order which they are
removed from the algorithm:
for the $k$-th removed interval $j_k \in \contain_i$,
at that time $\remainingcontainni$ is $\containni - k + 1$,
which guarantees that $\assign_{j_k}$ is at least $\containni - k + 1$.
Thus, \emph{Local Dominance} is satisfied.


\noindent\emph{\rom{2}. Global Dominance.}
%\paragraph{Global Dominance}
We prove this by induction. Consider the reverse order of intervals removed
from the remaining interval set $\remaining$ in the algorithm,
i.e., we set $\remaining = \emptyset$ as the base case and then add intervals back to $\remaining$
in the reverse order which they have been removed in the algorithm. 
Our induction hypothesis is that restricting to intervals in $\remaining$ the
\emph{Global Dominance} holds,
i.e., for any decreasing and concave function $\bar\pen$,
\begin{align}
\label{eq:global dominance}
\sum_{i\in \remaining} \bar\pen(\assign_i) \geq \sum_{i \in \remaining} \bar\pen(\remainingcontainni).
\end{align}

\emph{Base Case ($\remaining = \emptyset$):} In this case, the induction hypothesis holds trivially.

\emph{Inductive Step:}  Suppose the induction hypothesis holds before we add interval $i$ 
with $\assign_{i}$ back
to $\remaining$. 
Let $m = \assign_{i} - 1$.
To make it clear, let $\remaining$ to be the remaining interval set before we add interval $i$,
and $\remaining'$ to be the remaining interval set after we add interval $i$, i.e., 
$\remaining' = \remaining \cup\{i\}$.
%Let $\assign^{-1}(c) = |\{j \in W: \assign_j = c\}|$
%and 
%$\containn^{-1}(c) = |\{j \in W: |\contain_j \cap W| = c\}|$.
Next we consider the increment of both sides in 
\eqref{eq:global dominance}
after 
we add interval $i$ into $\remaining$.
The left hand side of \eqref{eq:global dominance} increases by $\bar\pen(m + 1)$.
%$\assign^{-1}(k)$ increases by one 
%while $\assign^{-1}(k')$ does not change for all $k' \not=k$.
For the right side, since $\assign_i = m + 1$,
there exist $m$ intervals $j_1, j_2, \dots j_m \in \remaining$
which 
%such that interval $j_k$ 
cover position $a_{\pmother_i}$,
and $i < j_k$ (otherwise, $j_k$ should be removed early than $i$ in the algorithm)
for all $k\in[m]$.
This implies that interval $i$ covers position $a_{j_k}$ 
for all $k \in[m]$.
Without loss of generality, we assume $j_1 < j_2 < \dots < j_m$,
then $
|\remainingcontain_{j_k}|\geq k$.
Hence, once we add interval $i$ into $W$,
the right hand side of \eqref{eq:global dominance}
increases by 
\begin{align*} 
&~~\bar\pen(|\contain_i^{\remaining'}|) + 
\sum_{j\in \remaining}
\left(
\bar\pen(|\contain_{j}^{\remaining'}|) - 
\bar\pen(|\contain_{j}^{\remaining}|)
\right) 
\leq \bar\pen(|\contain_i^{\remaining'}|) + 
\sum_{k\in[m]}
\left(
\bar\pen(|\contain_{j_k}^{\remaining'}|) - 
\bar\pen(|\remainingcontain_{j_k}|)
\right) \\
&=
\bar\pen(|\contain_i^{\remaining'}|) + 
\sum_{k\in[m]}
\left(\bar\pen(|\remainingcontain_{j_k}| + 1) - 
\bar\pen(|\remainingcontain_{j_k}|)\right) 
% \\
\overset{(a)}{\leq} 
\bar\pen(1) + 
\sum_{k \in [m]}
(
\bar\pen(k + 1) - \bar\pen(k)
)
= \bar\pen(m + 1)
\end{align*}
where (a) holds because $\bar\pen$ is decreasing and concave.
Applying the induction hypothesis (before we add interval $i$),
the inductive claim (after we add interval $i$) holds,
which finishes the induction.

\noindent\emph{\rom{3}. Partition Monotonicity.}
%\paragraph{Partition Monotonicity}
We first introduce the following two claims:
(a) for each interval $i\in[s]$, there is at most one interval $j$ such that
$\pfather_j = i$;
(b) for each interval $i\in[s]$ with $\assign_i > 1$, $\pfather_i \not= -1$.  
Note that claim (a) and (b) together imply that $\{\pfather_1, \dots, \pfather_s\}$ 
defines a partition which satisfies \emph{Partition Monotonicity} 
from \Cref{alg:partition monotonicity construction}.

Next, we show claim (a) and claim (b) separately.
We show claim (a) by contradiction. 
Suppose there exists interval $i$, $j_1$ and $j_2$ such that 
$\pfather_{j_1} = \pfather_{j_2} = i$.
By the construction of the algorithm,
$\assign_{j_1} = \assign_{j_2} = \assign_i + 1$.
Now, consider case by case.

\vspace{1.5mm}

\noindent\textbullet\ \emph{Case 1 ($i < j_1$ or $i < j_2$):} Without loss of generality, we assume $i < j_1$,
and the case $i < j_2$ is symmetric.
%Consider the moment when the algorithm 
%removes interval $j_1$ due to $\pmother_{j_1}$.
By the construction of the algorithm,
$\pfather_{j_1} = i$ implies 
$i \in \contain_{\pmother_{j_1}}$. 
%interavl $i$ also covers position $a_{\pmother_{j_1}}$,
This leads to a contradiction, because 
if $i < j_1$, interval $i$ should be removed early than interval $j_1$ in the algorithm 
which implies $\assign_i \geq \assign_{j_1}$.

\noindent\textbullet\ 
\emph{Case2 ($j_1, j_2 < i$):}

\hspace{5mm}\noindent\textbullet\ 
\emph{Case 2a ($\pmother_{j_1} < \pmother_{j_2}$ or $\pmother_{j_2} < \pmother_{j_1}$):}
W.L.O.G., we assume $\pmother_{j_1} < \pmother_{j_2}$ ($\pmother_{j_2} < \pmother_{j_1}$ is similar):

\hspace{10mm}\noindent\textbullet\ \
\emph{Case 2a1 (interval $j_1$ is removed before interval $j_2$):}
In this case, consider the moment 
when the algorithm removes $j_1$ due to interval $\pmother_{j_1}$.
By the construction of the algorithm, since $j_1$ is removed before $j_2$,
it implies
$|\remainingcontain_{\pmother_{j_1}}| > |\remainingcontain_{\pmother_{j_2}}|$.
Thus,
$\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
contradiction.

\hspace{10mm}\noindent\textbullet\ \
\emph{Case 2a2 (interval $j_2$ is removed before interval $j_1$):}
In this case, consider the moment 
when the algorithm remove $j_2$ due to interval $\pmother_{j_2}$.
Notice that interval $j_2$ also covers position $a_{\pmother_{j_1}}$,
i.e., $j_2 \in \contain_{\pmother_{j_1}}$.
By the construction of the algorithm, since $j_2$ is removed before $j_1$,
it implies
$|\remainingcontain_{\pmother_{j_1}}|  \leq |\remainingcontain_{\pmother_{j_2}}|$.
Thus, once the algorithm removed $j_2$, 
$|\contain_{\pmother_{j_1}}^{\remaining/\{j_2\}}|$ (which is an upper bound
of $\assign_{j_1}$) 
becomes strictly smaller than 
$|\remainingcontain_{\pmother_{j_2}}|$ (which is equal to $\assign_{j_2}$), %which 
%implies $\assign_{j_1}$ is strictly smaller than $\assign_{j_2}$,
contradiction.


\hspace{5mm}\noindent\textbullet\ 
\emph{Case 2b ($\pmother_{j_1} = \pmother_{j_2}$):}
Without loss of generality, we assume interval $j_1$ is removed before interval $j_2$,
and the case where interval $j_2$ is removed before interval $j_1$ is 
symmetric.
Let $\pmother^* = \pmother_{j_1} = \pmother_{j_2}$. Consider the moment
when the algorithm removes $j_1$ due to $\pmother^*$.
By the construction of the algorithm,
$\assign_{j_1} = 
|\remainingcontain_{\pmother^*}|$
and $\assign_{j_2} \leq |\contain_{\pmother^*}^{\remaining/\{j_1\}}|
= |\remainingcontain_{\pmother^*}| - 1$.
Thus, $\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
which is a contradiction.

\vspace{1.5mm}

We show claim (b) as follows. For any interval $i$
with $\assign_i > 1$,
consider the next removed interval $j$ %which covers 
%position $a_{q_i}$ and is the first interval removed 
among
$\contain_{\pmother_i}$ after the algorithm removes interval $i$.
It is sufficient to show $\assign_j = \assign_i - 1$,
which implies that algorithm set $\pfather_i = j$ when it removes interval $j$.
Since $j$ is the next interval removed among $\contain_{\pmother_i}$ after 
interval $i$, $\assign_i - 1\leq \assign_j \leq \assign_i$.
To show $\assign_j < \assign_i$, we use contradiction.
Suppose $\assign_j = \assign_i$. If $i\in\contain_{\pmother_j}$,
this implies that at the moment when the algorithm removes $i$, 
$
\assign_i = |\contain_{\pmother_i}^{\remaining}|
\geq
|\contain_{\pmother_j}^{\remaining}| \geq \assign_j + 1 = \assign_i + 1
$, contradiction.
If $i \not\in \contain_{\pmother_j}$, since $i < j$, 
it implies that $\pmother_i < \pmother_j$ and
at the moment when the algorithm removes $i$,
$|\contain_{\pmother_i}^\remaining|
=
\assign_i
=\assign_j 
\leq |\contain_{\pmother_j}^\remaining|
$, contradiction.
% \qedhere
\end{proof}

==> Paper/apx-IB-general-function.tex <==

\IBratio*
\begin{proof}
[Proof of \Cref{thm:concave competitive ratio}]
	Consider the following primal linear program, i.e., 
	\ref{eq:exante-adversarial-relax}:
	\begin{align*}
	\begin{array}{llll}
	{\max
	\limits_{\mathbf \alloc \geq \mathbf 0}}~&
	\displaystyle\sum\nolimits_{t=1}^\totaltime 
	\displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(t)}
	\displaystyle\sum\nolimits_{i=1}^n
	\reward_i\choice_t(\indexnew, i) \curalloc
	&\text{s.t.}& \\[1em]
	  \langle\theta_{i,k, t}\rangle
	  &
	\displaystyle\sum\nolimits_{\tpre = t}^{\min\{\totaltime,t+\duration_i-1\}}
	\displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(\tpre):
	(i, k)\in \indexnew}
	\choice_{\tpre}(\indexnew, i)
	\prealloc \leq 1
	& i \in [n],\ 
	k\in[\finalinventoryi],\
	t \in [\addtimeTilde(i, k): \totaltime]&
	\\[1em]
	  \langle\lambda_{t}\rangle
	&
	\displaystyle\sum\nolimits_{\indexnew \in \indexsetTilde(t)}
	\curalloc 
	\leq 1
	&t \in [\totaltime]&\\
	\intertext{We then construct its dual program with dual variables $\{\inventoryduali\}$ 
	and $\{\probduali\}$ as follows:} 
		\min
		\limits_{\boldsymbol{\theta},\boldsymbol{\lambda} \geq \mathbf 0} &
		\displaystyle\sum\nolimits%\limits
		_{i=1}^n
		\displaystyle\sum\nolimits%\limits
		_{k=1}^{\finalinventoryi}
		\displaystyle\sum\nolimits%\limits
		_{t=\addtimeTilde(i,k)}^\totaltime
		\inventoryduali
		+
		\displaystyle\sum\nolimits_{t =1}^\totaltime
		\probduali
		& 
		\text{s.t.} 
		&\\ 
	  \langle\curalloc\rangle
		&
		\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre} \vspace{1mm}
		\\
		&
		\qquad\qquad\qquad\qquad
		\qquad\qquad
		\geq \displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\reward_i\choice_t(\indexnew, i)
		& t \in [\totaltime],\ \indexnew \in \indexsetTilde(t)
		&
	\end{array}
\end{align*}	
	Let $\indexnew_t$ be the unit-specified assortment offered to consumer $t$.
	Recall $\curinventoryi$ 
	is the 
	inventory level of bin $j$ of  product $i$ at time period $t$ 
	before 
	the realization of 
	consumer $t$'s randomized choice.
For each product $i$ and bin $j$,
consider the following 
instance of the Interval Assignment Problem (IAP)
in \Cref{def:IAP}
separately.
Let 
%it has been allocated at time 
$\texttt{alloc}_{i}^{j} = \{t_1, t_2, \dots, t_s\}$
be the time periods when a unit of product $i$ from 
$\batch_{i, j}$ 
is selected.
Consider the instance of IAP with $s$ intervals
$\{[t_1, t_1 + \duration_i], \dots, 
[t_s, t_s + \duration_i]\}$.
Let 
$\{\assign_{i,j, t}\}_{t\in \texttt{alloc}_{i}^{j}}$ 
be the assignment solved in IAP for bin $j$ of product $i$
and let 
$\pseudoinventory_{i, j, t} = 
|\batch_{i}^{j}| - \assign_{i,j, t}$ 
if $t \in \texttt{alloc}_{i}^{j}$
and $\pseudoinventory_{i,j, t} = 1$ otherwise.

    Consider the following assignments of primal (which is deterministic) and 
    % $\{\probduali\}$ in 
    dual (which is randomized):
	\begin{align*}
		\textit{Primal:}~\curalloc &= \indicator{\indexnew_t = \indexnew},\\
		&&&\\
		\textit{Dual:}~~~ \probduali &= 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew_t}
		\reward_i 
		\pen\left(
		\frac{\curinventory_{i, t}^{\batchid}}
    {|\batch_{i}^{\batchid}|}
		\right)
		\cdot
			\indicator{\text{a unit  
			from $\batch_{i}^{\batchid}$
			is selected at time $t$}} \\
			\inventoryduali &= 
			\reward_i\left(
			\pen\left(
		\frac{\pseudoinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
			\right) -
			\pen\left(
\frac{\pseudoinventory_{i, t}^{\batchidTilde}-1}
    {|\batch_{i}^{\batchidTilde}|}
			\right)
			\right) 
% 			\\
% 			&
% 			~~~~~~~~~~~~
% 			~~~~~~
			\cdot
			\indicator{\text{a unit  
			from $\batch_{i}^{\batchidTilde}$
			is selected at time $t$}}~.
	\end{align*}
	where 
		$\indicator{\cdot}$ is an indicator operator. 
		Note that product $i$ is selected at time $t$ 
		if it belongs to the unit-specified assortment 
		set $\indexnew_t$ 
		and 
		consumer arriving at time $t$ chooses this product.  
	Note that for any product $i$ and unit $k$,
	by construction we have
	$\batchidTilde \leq 
	\cnt_{i, \addtimeTilde(i,k)} - 1$,
	i.e., 
	batch $\batch_{i,\batchidTilde}$
	is created no later 
	than time $\addtimeTilde(i,k)$.
	Thus, 
	$\pseudoinventory_{i,t}^{\batchidTilde}$ 
	and $\inventorydual_{i,k,t}$
	are well-defined 
	for any time $t\geq \addtimeTilde(i,k)$.
	
		In the rest of analysis, we show the above randomized primal-dual assignments satisfy the conditions of \Cref{lem:random primal-dual} for 
		$\Gamma(\pen, \gamma)$,
		which finishes the proof.
	\vspace{1mm}

	\noindent\emph{\rom{1}. Primal feasibility and dual feasibility in expectation.}
 The primal assignment is feasible, as 
 \IBB\ only offers inventory feasible assortments. 
 To show dual feasibility in expectation, 
 first note that $\pen(\cdot)$ is non-negative and monotone non-decreasing. 
 Therefore $\probduali\geq 0$ for all $t\in[\totaltime]$, and $\inventoryduali\geq 0$ for all 
 $i\in[n],k\in[\finalinventoryi],t\in[\addtimeTilde(i,k):\totaltime]$. 
 Next, we show for every $t\in[\totaltime]$ and
 $\indexnew\in\indexsetTilde(t)$, 
 the dual assignment satisfies the dual constraints corresponding to $\curalloc$ in expectation. 
 %Let $\indicator{\duration_{i, \tpre} \geq t - \tpre}$ be the indicator of the event that rental time of product $i$ at time $\tpre$ is at least 
	%$t - \tpre$. 
	For every product $i$ and unit $k$, 
	the following inequality holds at every time 
	$t\in[\addtimeTilde(i,k):\totaltime]$: 
	\begin{align}
		\label{eq:dual feasible ex post general}
		\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-\duration_i + 1, \addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre} 
		\geq \reward_i
	\end{align}
	To see why 
	inequality~\eqref{eq:dual feasible ex post} holds, 
	consider on-hand units and not returned 
	units of product $i$ 
	in bin $\batch_{i}^{\batchidTilde}$
	at time $t$. 
	Since the inventory level of bin
	$\batch_{i}^{\batchidTilde}$
	at time $t$ is 
	$\curinventory_{i,t}^{\batchidTilde}$, 
	there are $m \triangleq
	|\batch_{i}^{\batchidTilde}| 
	-
	\curinventory_{i,t}^{\batchidTilde}$ 
	units of product $i$ from this bin
	not returned at that moment. 
	Suppose these units were rented at times
	$\tpre_1\leq\tpre_2\leq
	\dots\leq\tpre_{m}$,
	where $\max\{t-\duration_i + 1, \addtimeTilde(i,k)\}
	\leq \tpre_\ell \leq t - 1$ 
% 	and 
% 	$\indicator{\text{a unit of product $i$ 
% 			from $\batch_{i,\batchidTilde}$
% 			is selected at time $\tpre_\ell$}}=1$
% 	for all $\ell\in[m]$.
	Additionally, recall 
$\{\assign_{i,t}^{\batchidTilde}\}_{t\in \texttt{alloc}_{i}^{\batchidTilde}}$ is assignment in IAP which satisfies
\emph{Local Dominance}.
By Local Dominance at interval starting at $\tpre_{m}$,
there exists a bijection $\rho_{i,\tpre_m}^{\batchidTilde}$ from $\contain_{i,\tpre_{m}}^{\batchidTilde}$
to $\{1,2,\dots,|\contain_{i,\tpre_{m}}^{\batchidTilde}|\}$ such that 
$\assign_{i,\tpre}^{\batchidTilde}
\geq \rho_{i,\tpre_m}^{\batchidTilde}(\tpre)$ for all $\tpre \in \contain_{i,\tpre_{m}}^{\batchidTilde}$.
Notice that intervals starting at 
$\tpre_1, \tpre_2, \dots \tpre_{m}$
all cover time $\tpre_{m}$,
i.e.,
$\tpre_\ell \in \contain_{i,\tpre_{m}}^{\batchidTilde}$ 
for all 
$\ell\in[m]$.
Thus, we can construct
bijection $\rho_{i,t}^{\batchidTilde}$ from
$[m]$
to $[m]$
such that
$\assign_{i,\tpre_\ell}^{\batchidTilde} \geq
\rho_{i,t}^{\batchidTilde}(\ell)$
for all $\ell \in [m]$.
Because the penalty function $\pen(\cdot)$ is concave and increasing,
\begin{align}
\begin{split}
\label{eq:concave general}
\theta_{i, k, \tpre_\ell} &= 
\reward_i\left(
\pen\left(\frac{
\pseudoinventory_{i,\tpre_\ell}^{
\batchidTilde}}{|\batch_{i}^{\batchidTilde}|}\right)
-
\pen\left(\frac{\pseudoinventory_{i,\tpre_\ell}^{
\batchidTilde}-1}{|\batch_{i}^{\batchidTilde}|}\right)
\right)  \\
&=
\reward_i\left(
\pen\left(\frac{|\batch_{i}^{\batchidTilde}| - 
\assign_{i,\tpre_\ell}^{
\batchidTilde}}{|\batch_{i}^{\batchidTilde}|}\right)
-
\pen\left(\frac{
|\batch_{i}^{\batchidTilde}|-
\assign_{i,\tpre_\ell}^{
\batchidTilde}-1}{|\batch_{i}^{\batchidTilde}|}\right)
\right)  \\
&\geq
\reward_i\left(
\pen\left(\frac{|\batch_{i}^{\batchidTilde}| - \rho_{i,t}^{\batchidTilde}(\ell)}
{|\batch_{i}^{\batchidTilde}|}\right)
-
\pen\left(\frac{|\batch_{i}^{\batchidTilde}| - \rho_{i,t}^{\batchidTilde}(\ell)- 1}{|\batch_{i}^{\batchidTilde}|}\right)
\right)
\end{split}
\end{align}
By applying \eqref{eq:concave general},  we can prove inequality~\eqref{eq:dual feasible ex post general}:
\begin{align*}
&\quad~
\reward_i
		\pen\left(
		\frac{\curinventory_{i, t}^{\batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-\duration_i + 1, \addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre} 
		\\
		& 
		\geq
		\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{ \batchidTilde}}
    {|\batch_{i}^{ \batchidTilde}|}
		\right) 
		+ 
		\displaystyle\sum\nolimits_{\ell = 1}^{m} 	\reward_i\left(
		\pen\left(
		\frac{
		\pseudoinventory_{i,
		\tpre_\ell}^{\batchidTilde}
		}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		-
	\pen\left(
		\frac{
		\pseudoinventory_{i,
		\tpre_\ell}^{\batchidTilde} - 1
		}
		{|\batch_{i}^{\batchidTilde}|}
	\right)
	\right) 
	\\
		&\geq
			\reward_i
		\pen\left(
		\frac{\curinventory_{i, t}^{\batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+
		\displaystyle\sum\nolimits_{\ell = 1}^{m}\reward_i\left(
		\pen\left(
		\frac{|\batch_{i}^{\batchidTilde}| 
		- \rho_{i,t}^{\batchidTilde}(\ell)}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		-
	\pen\left(
	\frac{
	|\batch_{i}^{\batchidTilde}| - \rho_{i,t}^{\batchidTilde}(\ell)-1}
	{|\batch_{i}^{\batchidTilde}|}\right)
	\right)
	\\
	&=
	\reward_i
		\pen\left(
		\frac{\curinventory_{i, t}^{\batchidTilde}}
    {|\batch_{i}^{\batchidTilde}|}
		\right) 
		+
	\displaystyle\sum\nolimits_{I = \curinventory_{i,t}
	^{\batchidTilde}}^{
	|\batch_{i}^{\batchidTilde}| - 1
	} 
		\reward_i\left(
			\pen\left(\frac{I}{|\batch_{i}^{ \batchidTilde}|}\right) 
			-
			\pen\left(\frac{I-1}{|\batch_{i}^{ \batchidTilde}|}\right) 
		\right)\\
		&
		\geq\reward_i\pen(1)=\reward_i
\end{align*}	

Now, for each time $t\in[\totaltime]$ 
and 
unit-specified assortment 
$\indexnew\in\indexsetTilde(t)$, consider the following expression:
	\begin{align}
		\label{eq:dual LHS general}
	\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}
	\end{align}
On the one hand, note that by taking expectation from \eqref{eq:dual LHS general} we have 
\begin{equation}
\begin{split}
\label{eq:first-compare general}
&\expect{
	\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}
		}\\
		=&\expect{\probduali} + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)
		\expect{\theta_{i,k,\tpre}} ~,
		\end{split}
\end{equation}
simply because of linearity of expectation. 
On the other hand, by taking expectation 
from $\probduali$
% \eqref{eq:dual LHS} 
by first conditioning on (i) history up to time $t$ (which includes inventory levels $\curinventory_{i,t}^{j}$ for each product $i$, bin $j$), 
and 
(ii) unit-specified assortment $\indexnew_t$ 
offered at time $t$, we have
\begin{align}
\label{eq:lambda conditional lowerbound general} 
\begin{split}
\expect{
		\probduali  \condition\mathcal{F}_{t-1},\indexnew_t
		}
		&=
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew_t}
		\reward_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchid(i,k)}}
		{|\batch_{i}^{\batchid(i,k)}|}
		\right)
		\\
		&\overset{(a)}{=}
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew_t}
		\reward_i\choice_{t}(\indexnew_t, i)
		\pen\left(
		\inventoryratio_{i, t}^{\batchid}
		\right)
		\\
		&\overset{(b)}{\geq} 
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew}
		\reward_i\choice_{t}(\indexnew , i)
		\pen\left(
		\inventoryratio_{i, t}^{\batchidTilde}
		\right)
		\\
		&\overset{(c)}{=}
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew}
		\reward_i\choice_{t}(\indexnew, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		\end{split}
\end{align}
where $\mathcal{F}_{t-1}$ 
denotes the history up to time $t$.
% and $\indexnew'$ is a unit-specified assortment 
% satisfying that $(i, k')\in \indexnew'$
% if and only if there exists
% $(i, k) \in \indexnew$ such that
% $\batchid(i,k')=\batchidTilde$.
Inequality~(a)  holds since 
for all $(i,k) \in \indexnew_t$
we have
$\batchid< \cnt_{i,t}$ and thus
$\inventoryratio_{i,t}^{\batchid} = 
\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}
		\cdot 
		\indicator{\batchid<\cnt_{i,t}}
		=\frac{\curinventory_{i,t}^{\batchid}}
		{|\batch_{i}^{\batchid}|}$;
		inequality~(c) holds for a similar reason;
		and
	inequality~(b) holds since 
	\begin{align*}
	    \indexnew_t
	    \in
	     \argmax\limits_{
    \indexnew\in \indexset(t)}
    \sum_{(i, k)\in \indexnew} 
    \reward_i\choice_{t}(\indexnew, i)
    \pen\left(\inventoryratio_{i,t}^{\batchid(i,k)}\right)
    \cdot 
    \indicator{
    \text{unit $k$ of product $i$ is available}}~.
	\end{align*}
	Now consider
	the expectation of 
	\eqref{eq:dual LHS general} 
	conditioning on 
	$\mathcal{F}_{t-1},\indexnew_t$,
	\begin{align*}
		&\expect{
		\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre} \condition\mathcal{F}_{t-1},\indexnew_t
		}\nonumber\\
		&~~\overset{(a)}{\geq}
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew}
		\reward_i\choice_{t}(\indexnew, i)
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
		{|\batch_{i}^{\batchidTilde}|}
		\right)
		+	
		\displaystyle\sum\nolimits_{(i,k)\in 
		\indexnew}
		\displaystyle\sum\nolimits_{\tpre =
		\max\{t-\duration_i+1,\addtimeTilde(i,k)\}}^{t - 1}
		\choice_t(\indexnew,i) 
		\inventorydual_{i,k, \tpre} \nonumber \\
		&~~=
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew} 
		\choice_{t}(\indexnew,i)
		\left(\reward_i
		\pen\left(
		\frac{\curinventory_{i,t}^{\batchidTilde}}
		{|\batch_{i}^{\batchidTilde}|}
		\right)+ \displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,\addtimeTilde(i,k)\}}^{t - 1}
		\inventorydual_{i,k, \tpre}  \right)
		\nonumber \\
		&~~\overset{(b)}{\geq} \displaystyle\sum\nolimits_{(i,k)\in\indexnew} 
		\reward_i\choice_t(\indexnew,i)~,\nonumber
	\end{align*}
where
inequality~(a) holds by 
applying inequality~\eqref{eq:lambda conditional lowerbound general}
and dropping non-negative terms related to 
$\inventorydual_{i,k,t}$ for all $(i,k)\in \indexnew$;
and 
inequality~(b) holds because of  inequality~\eqref{eq:dual feasible ex post general}. Therefore, by taking another expectation over $\indexnew_t$ and  $\mathcal{F}_{t-1}$, we have:
\begin{equation}
\label{eq:second-compare general}
\expect{
\probduali + 
		\displaystyle\sum\nolimits_{(i,k)\in \indexnew}
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, \addtimeTilde(i,k)\}}^t
		\choice_t(\indexnew,i)\theta_{i,k,\tpre}
		}\geq \displaystyle\sum\nolimits_{i = 1}^n 
		\reward_i\choice_t(\indexnew,i)
\end{equation}
Combining \eqref{eq:first-compare general} and \eqref{eq:second-compare general} shows feasibility in expectation of the dual assignment.

\noindent\emph{\rom{2}. Comparing objective values of primal and dual.}
Fix an arbitrary product $i$ and bin $j$,
we consider the contribution of $\batch_{i}^{j}$ in primal vs.\ 
$\batch_{i}^{j}$ for $\{\probduali\}$ 
and $\batchTilde_{i}^{j}$ for $\{\inventoryduali\}$ in dual 
(i.e., $\text{Primal}_{i}^{j}$ and $\text{Dual}_{i}^{j}$)
at each sample path 
separately.
Recall $\texttt{alloc}_{i}^{j}$
is the set of time periods when
a unit from $\batch_{i}^{j}$ has been selected,
\begin{align*}
\text{Primal}_{i}^{j} &= 
\reward_i
\displaystyle\sum\nolimits_{t = 1}^\totaltime
\indicator{\text{a unit from $\batch_{i}^{j}$ is selected at time $t$}}
\\
&= \reward_i|\texttt{alloc}_{i}^{j}| \\
\text{Dual}_{i}^{j} &= 
\reward_i
\displaystyle\sum\nolimits_{t = 1}^\totaltime 
\left(
\pen\left(
\frac{\curinventory_{i,t}^{j}}{|\batch_{i}^{j}|}
\right) 
+
|\batchTilde_{i}^{j}|\left(
\pen\left(
\frac{\pseudoinventory_{i,t}^{j}}{|\batch_{i}^{j}|}
\right) 
-
\pen\left(
\frac{\pseudoinventory_{i,t}^{j} - 1}{|\batch_{i}^{j}|}\right) 
\right)
\right)\\
&~~~~~~~~~~~
\qquad\qquad
\cdot \indicator{\text{a unit from $\batch_{i}^{j}$ is selected at time $t$}} \\
&=
\reward_i
\displaystyle\sum\nolimits_{t \in \texttt{alloc}_{i}^{j}} 
\left(
\pen\left(\frac{\curinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right) 
+
|\batchTilde_{i}^{j}|\left(
\pen\left(\frac{\pseudoinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right) 
-
\pen\left(\frac{\pseudoinventory_{i,t}^{j} - 1}{|\batch_{i}^{j}|}\right) \right)
\right)
\end{align*}
Consider decreasing and concave function $\bar\pen(x) = \pen(1 - x)$,
by \emph{Global Dominance} of IAP assignment,
\begin{align*}
\sum_{t\in \texttt{alloc}_{i}^{j}}
	\pen\left(\frac{\pseudoinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right)  
	&=
\sum_{t\in \texttt{alloc}_{i}^{j}}
	\pen\left(\frac{|\batch_{i}^{j}| - 
	\assign_{i, t}^{j}}{|\batch_{i}^{j}|}\right)   
	=
\sum_{t\in \texttt{alloc}_{i}^{j}}
\bar\pen\left(\frac{ \assign_{i,t}^{j}}{|\batch_{i}^{j}|}\right)  
\\
&\geq 
\sum_{t\in \texttt{alloc}_{i}^{j}}
\bar\pen\left(\frac{|\batch_{i}^{j}| - \curinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right)   
	=
\sum_{t\in \texttt{alloc}_{i}^{j}}
	\pen\left(\frac{\curinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right)   
\end{align*}
Hence,
\begin{align*}
\text{Dual}_{i}^{j} &\leq 
\reward_i
\displaystyle\sum\nolimits_{t \in \texttt{alloc}_{i}^{j}} 
\left(
\pen\left(\frac{\pseudoinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right) 
+
|\batchTilde_{i}^{j}|\left(
\pen\left(\frac{\pseudoinventory_{i,t}^{j}}{|\batch_{i}^{j}|}\right) 
-
\pen\left(\frac{\pseudoinventory_{i,t}^{j} - 1}{|\batch_{i}^{j}|}\right) \right)
\right)
\end{align*}
Now, we partition time periods in $\texttt{alloc}_{i}^{j}$ 
into subgroups 
$A_{i}^{j, 1}, A_{i}^{j, 2}, \dots, A_{i}^{j, \kappa}$ 
defined by \emph{Partition Monotonicity}
of IAP assignment, and consider the contribution of each subgroup $A_{i}^{j, \ell}$ in primal and dual 
(i.e. $\text{Primal}_{i}^{j, \ell}$ and 
$\text{Dual}_{i}^{j, \ell}$)
separately.
Recall that \emph{Partition Monotonicity} guarantees that 
$\{\assign_{i,t}^{j}:t \in A_{i}^{j, \ell}\} 
= \{1, 2, \dots, |A_{i}^{j,\ell}|\}$,
thus,
$\{\pseudoinventory_{i,t}^{j}:t \in A_{i}^{j,\ell}\} 
= \{|\batch_{i}^{j}| - |A_{i}^{j,\ell}| + 1, 
|\batch_{i}^{j}| - |A_{i}^{j,\ell}| + 2, 
\dots, |\batch_{i}^{j}|\}$.
Thus, let $x_{i}^{j,\ell} = \frac{|\batch_{i}^{j}| - 
|A_{i}^{j,\ell}|}{|\batch_{i}^{j}|}$,
\begin{align*}
\text{Primal}_{i}^{ j,\ell} &= 
\reward_i (1-x_{i}^{j,\ell})|\batch_{i}^{j}|  \\
\text{Dual}_{i}^{j,\ell} 
&\leq 
\reward_i \sum_{I = x_{i}^{j,\ell}\,|\batch_{i}^{j}|  + 1}^{|\batch_{i}^{j}|}
\left(
\pen\left(\frac{I}{|\batch_{i}^{j}|}\right) 
+
|\batchTilde_{i}^{j}|\left(
\pen\left(\frac{I}{|\batch_{i}^{j}|}\right) 
-
\pen\left(\frac{I- 1}{|\batch_{i}^{j}|}\right) \right)
\right) \\
&= 
\reward_i 
\sum_{I = x_{i}^{j,\ell}\,|\batch_{i}^{j}|  + 1}^{|\batch_{i}^{j}|}
\pen\left(\frac{I}{|\batch_{i}^{j}|}\right) 
+
\reward_i|\batchTilde_{i}^{j}|\left(
\pen(1) - 
\pen\left(x
%\frac{x}{|\batch_{i}^{j}|}
\right)
\right)
\end{align*}
Since $\pen(1) = 1$ and $\pen$ is increasing, it implies
\begin{align*}
\sum_{I = x_{i}^{j,\ell}\,|\batch_{i}^{j}|  + 1}^{|\batch_{i}^{j}|}
\pen\left(\frac{I}{|\batch_{i}^{j}|}\right) 
&=
1 + 
\sum_{I = x_{i}^{j,\ell}\,|\batch_{i}^{j}|  + 1}^{|\batch_{i}^{j}| - 1}
\pen\left(\frac{I}{|\batch_{i}^{j}|}\right) \leq 
1 + 
\int_{x_{i}^{j,\ell}+\frac{1}{|\batch_{i}^{j}|}}^1
\pen(y)\,dy
\end{align*}
Thus,
\begin{align*}
\text{Dual}_{i}^{ j,\ell} &\leq 
\reward_i|\batch_{i}^{j}|\left(
\frac{1}{|\batch_{i}^{j}|} + \int_{x_{i}^{j,\ell}
+\frac{1}{|\batch_{i}^{j}|}}^1
\pen(y)\,dy
+
\frac{|\batchTilde_{i}^{j}|}{|\batch_{i}^{j}|}
\left(1 -
\pen\left(
x
\right)
\right)
\right)
\end{align*}
and
\begin{align*}
\frac{\text{Primal}_{i}^{ j,\ell}}
{\text{Dual}_{i}^{j,\ell}} 
&\geq
\frac{1 - x_{i}^{j,\ell}}
{
\frac{1}{|\batch_{i}^{j}|} + \int_{x_{i}^{j,\ell}+\frac{1}{|\batch_{i}^{j}|}}^1
\pen(y)\,dy
+
\frac{|\batchTilde_{i}^{j}|}{|\batch_{i}^{j}|}
\left(1 -
\pen\left(
x
\right)
\right)
}
\end{align*}
Note that $|\batch_{i}^{j}| \geq \inventory_i\geq \mininventory$,
$\frac{|\batchTilde_{i}^{j}|}{|\batch_{i}^{j}|} \leq (1 + \gamma)$
for $j = 1$; 
and $|\batch_{i}^{j}| \geq \gamma\inventory_i
\geq  \gamma\mininventory$,
$\frac{|\batchTilde_{i}^{j}|}{|\batch_{i}^{j}|} \leq 1$
for $j > 1$.
Thus,
we finish showing that 
\begin{align*}
\frac{\text{Primal}}
{\text{Dual}} 
&\geq
\min_{i \in [n],j\in [\cnt_{i,T}]}
\frac{\text{Primal}_{i,j}}
{\text{Dual}_{i,j}}  
\geq
\min_{i \in [n]}
\min_{A_{i}^{j,\ell}}
\frac{\text{Primal}_{i}^{ j,\ell}}
{\text{Dual}_{i}^{j,\ell}}   
\geq
\Gamma(\pen, \gamma).
\end{align*}
Invoking \Cref{lem:tilde relaxation} and \Cref{lem:random primal-dual} finishes the proof.
\end{proof}



==> Paper/apx-dependent-fee-duration.tex <==
In this section, we consider 

==> Paper/apx-non-optimal-IB.tex <==


\label{apx:nuemrical-examples}
In this section, we discuss three natural modifications of \IB\ and show that they cannot achieve the optimal asymptotic competitive ratio $(1-\sfrac{1}{e})$ even if initial inventories are large and there is no endogenous inventory shock. Throughout this section, we assume that there are only exogenous shocks but no endogenous shock (i.e., $\duration_i = \infty$ for every product $i$).

\Cref{alg:IB} is the \IB\ (IB) algorithm introduced in \citet{GNR-14} for cases where there is no inventory shock. It can be verified that the \IBB\ algorithm is equivalent to IB in the absence of inventory shocks.

\input{Paper/alg-IB}

When there are exogenous inventory shocks, three natural generalizations of the IB algorithm can be considered:
\begin{itemize}
    \item \emph{\CNUIB}: In this generalization of the IB algorithm, for each time period $t$ and product $i$, the marginal revenue of all its units is discounted by the same factor of $\pen\left(\min\{\sfrac{\curinventory_{i, t}}
    {\inventory_i}, 1\}
    \right)$. Here $\curinventory_{i, t}$ is the inventory level of product $i$ at time period $t$. See \Cref{alg:CNUIB} for its formal description.
    \item \emph{\CUIB}: In this generalization of the IB algorithm, for each time period $t$ and product $i$, the marginal revenue of all its units is discounted by the same factor of $\pen\left(\sfrac{\curinventory_{i, t}}
    {(\inventory_i+\sum_{\tpre\in[t]}\replen_{i,\tpre}}
    )\right)$. Here $\curinventory_{i, t}$ is the inventory level of product $i$ at time period $t$, and $\replen_{i,t}$ is the new units of product $i$ added due to exogenous shocks. See \Cref{alg:CUIB} for its formal description.
    \item \emph{\UDIB}: In this generalization of the IB algorithm, each new unit of each product added due to exogenous shocks are treated as a new type of products. This is equivalent to the IBB algorithm (\Cref{alg:IBB}) with batch size threshold $\batchsizethreshold = 1$ (which automatically does not distinguish between ``charging'' and ``ready'' batches as well).
\end{itemize}
In \Cref{prop:non optimal IB}, we show that using exponential penalty function $\pen(x) = \frac{e^{1-x}-e}{1-e}$, all three generalizations of the IB algorithm above has strictly worse competitive ratio than the BIB algorithm, even when the minimum initial inventory $\mininventory$ are large.


\input{Paper/alg-CNUIB}
\input{Paper/alg-CUIB}

\begin{proposition}
\label{prop:non optimal IB}
    For exponential penalty function $\pen(x) = \frac{e^{1-x}-e}{1-e}$, the competitive ratios of \Cref{alg:CNUIB}, \Cref{alg:CUIB}, and \Cref{alg:IBB} with $\batchsizethreshold = 1$ is at most 0.552, 0.53, and 0.5, respectively, even as the smallest initial inventory $\mininventory$ goes to infinity.
\end{proposition}
\begin{proof}{\textsl{Proof.}}
We analyze the competitive ratios of all three algorithms separately. For each algorithm, we upper bound its competitive ratio by constructing an online bipartite matching instance, i.e., the special case of online assortment where choice model $\choice(\assortment, i) \in \{0, 1\}$ and $\choice(\assortment, i) = 1$ only if $\assortment = \{i\}$. 

\xhdr{Analyzing \CNUIB:} Our constructed instance $\matchinginstance(N, \reward, \supply)$ is parameterized by $N \in \naturals$ and $r, s\in[0, 1]$. In this instance, there are $N + 1$ product subgroups $\{\supplies_{\ell}\}_{\ell\in[0:N]}$, indexed by $[0: N]$. Each product subgroup $\supplies_{\ell}$ with $\ell\in[0:N]$ contains $n_\ell$ products, and each product $i$ in subgroup $\supplies_\ell$ has identical per unit price $\reward_i \triangleq \reward^\ell$ and identical initial inventory $\inventory_i \triangleq \inventory$. Here $\inventory$ is a large enough constant. On the other side, there are $2N + 1$ consumer subgroups $\{\demands_k\}_{k\in[0:2N]}$ indexed by $[0: 2N]$. Each consumer subgroup $\demands_k$ with $k\in[0:2N]$ contains $m_k$ consumers, who arrive sequentially.

Consumer subgroup $\demands_0$ has size $m_0 \triangleq \inventory \cdot n_0$. For each $i\in[n_0]$ and each time period $t\in [(i - 1)\inventory + 1:i\inventory]$, a new consumer from subgroup $\demands_0$ who accepts every product from $[n_0 - i + 1] \subseteq \supplies_0$ (i.e., the first $n_0 - i + 1$ products of $\supplies_0$) arrives. 

All remaining consumer subgroups $\{\demands_k\}_{k\in[2N]}$ and products subgroups $\{\supplies_k\}_{\ell\in[N]}$ are constructed recursively based on the execution of \CUIB.\footnote{Since the algorithm is deterministic, it suffices for us to construct instance $\matchinginstance(N, \reward, \supply)$ adaptively, based on the execution of the algorithm.} Specifically, for each $\ell\in[N]$,
\begin{itemize}
    \item Consider time period $t_\ell \triangleq \sum_{k\in[0:2(\ell-1)]}m_k$, i.e., the time period when the first consumer from consumer subgroup $\demands_{2\ell - 1}$ arrives. Let $x_{i, t_\ell}$ be the number of available units of product $i\in\supplies_{\ell - 1}$ at the beginning of time period $t_\ell$ in the algorithm. For each product $i\in\supplies_{\ell - 1}$, there are $\replen_{i,t_\ell} \triangleq \max\{\supply\cdot \inventory - x_{i,t_\ell},0\}$ new units added due to the exogenous inventory shocks. As a sanity check, for each product $i\in\supplies_{\ell-1}$ with $\replen_{i,t_{\ell}} > 0$, its inventory level becomes $\supply\inventory$ and has a discount factor of $\pen(\supply)$ in the algorithm.
    With slight abuse of notation, let $\replen_\ell\triangleq \sum_{i\in\supplies_{\ell - 1}}\replen_{i, t_\ell}$ be the total number of new units added for products from product subgroup $\supplies_{\ell - 1}$. 
    \item Product subgroup $\supplies_{\ell}$ has size $n_{\ell} \triangleq \frac{\replen_\ell}{\inventory\cdot \left(1 - \pen^{-1}\left(\frac{\pen(\supply)}{\reward}\right)\right)}$, where $\pen^{-1}$ is the inverse function of penalty function $\pen$.\footnote{In the construction of instance $\matchinginstance(N, \reward,\supply)$, we impose the requirement that $\frac{\pen(\supply)}{\reward}\in[0, 1]$ for parameters $\reward,\supply\in[0, 1]$. Note that under this requirement, together with the assumption that penalty function $\pen$ is exponential function, the inverse function $\pen^{-1}$ and $n_{\ell}$ are well-defined.} 
    \item Consumer subgroup $\demands_{2\ell - 1}$ have size $m_{2\ell- 1}\triangleq \replen_{\ell}$. For each new unit added for products from product subgroup $\supplies_{\ell-1}$ at time period $t_\ell$ due to exogenous shocks, there is a consumer in consumer subgroup $\demands_{2\ell-1}$ who accepts product $i\in\supplies_{\ell - 1}$ of this unit and one product $i'\in\supplies_{\ell}$. Here product $i'$ is constructed such that for each product $i'\in\supplies_{\ell}$, there are exactly $\frac{\replen_\ell}{n_{\ell}}$ consumers from $\demands_{2\ell - 1}$ accepts this product. Under this construction, for each consumer in $\demands_{2\ell - 1}$, suppose she accepts product $i\in \supplies_{\ell - 1}$ and product $i'\in \supplies_{\ell}$, the algorithm allocates product $i'\in\supplies_{\ell}$ to her and collects price $r^\ell$, since the discounted price of product $i'\in\supplies_{\ell}$ is larger than the discounted price of product $i\in\supplies_{\ell - 1}$ due to the construction of $n_\ell$. More specifically, note that the inventory level of product $i'$ when serving this consumer is at least $\inventory - \frac{\replen_\ell}{n_\ell}$. Thus, the discounted price of product $i'$ is at least 
    \begin{align*}
        \reward_{i'}\pen\left(1 - \frac{\replen_\ell}{\inventory\cdot n_\ell}\right)
        =
        \reward^\ell \pen\left(1 - \frac{\replen_\ell}{\inventory\cdot n_\ell}\right)
        =
        \reward^\ell \frac{\pen(\supply)}{\reward}
        =
        \reward^{\ell - 1}\pen(\supply)
        =
        \reward_{i}\pen(\supply)
    \end{align*}
    where the first and last equalities hold due to the construction of $\reward_{i}, \reward_{i'}$ from subgroups $\supplies_{\ell - 1},\supplies_{\ell}$; and the second equality holds due to the construction of $n_\ell$. Because of this allocation in the algorithm, after serving all consumers from consumer subgroup $\demands_{2\ell - 1}$, the inventory level of each product from product subgroup $\supplies_{\ell}$ is the same, which is equal to $\inventory - \frac{\replen_\ell}{n_\ell}$.
    \item Consumer subgroup $\demands_{2\ell}$ has size $m_{2\ell}\triangleq \inventory \cdot n_\ell$. For the $i$-th consumer in consumer subgroup $\demands_{2\ell}$, she accepts the first $n_\ell - \lfloor\frac{i}{\inventory}\rfloor$ products of product subgroup $\supplies_\ell$.
\end{itemize}
The clairvoyant optimum policy assigns a perfect matching between consumer subgroup $\demands_{2\ell}$ and product subgroup $\supplies_{\ell}$ for every $\ell\in[0:N]$, and assigns every consumer from consumer subgroup $\demands_{2\ell - 1}$ with a unit of her acceptable product from product subgroup $\supplies_{\ell - 1}$ that is added at time period $t_\ell$ due to exogenous shocks for every $\ell\in[N]$. Hence, the total revenue of the clairvoyant optimum policy is $\sum_{\ell\in[0:N]}\reward^\ell\cdot \inventory\cdot n_{\ell} + \sum_{\ell\in[N]}\reward^{\ell - 1}\cdot \replen_\ell$.

On the other end, \CNUIB\ is sub-optimal because of the revenue loss from two parts. First, it only assigns an imperfect matching between consumer subgroup $\demands_{2\ell}$ and product subgroup $\supplies_{\ell}$ for every $\ell\in[0:N]$. Moreover, for every $\ell\in[N]$ and every consumer from consumer subgroup $\demands_{2\ell - 1}$, the algorithm allocates a unit of her acceptable product from product subgroup $\supplies_{\ell}$. 

Based on the aforementioned instance construction, we numerically evaluate the performance \CNUIB\ on instance $\matchinginstance(20, 0.5, 0.32)$ with $n_0 = 500$, sufficiently large $\inventory$ and obtain a competitive ratio upper bound of 0.55106.

\xhdr{Analyzing \CUIB:} Our constructed instance $\hat\matchinginstance(N, \reward, \supply)$ is parameterized by $N \in \naturals$ and $r, s\in[0, 1]$. The construction of $\hat\matchinginstance(N, \reward, \supply)$ is almost the same as $\matchinginstance(N, \reward, \supply)$ above, expect that we set $\replen_{i,t_\ell}\triangleq \frac{\supply\cdot \inventory - x_{i,t_\ell}}{1-\supply}$ for every $\ell\in[N]$ and $i\in\supplies_{\ell - 1}$. Under this modification of $\{\replen_{i,t_\ell}\}$, we still ensure that for every $\ell\in[N]$ and every consumer from consumer subgroup $\demands_{2\ell - 1}$, \CUIB~ allocates a unit of her acceptable product from product subgroup $\supplies_{\ell}$, while the clairvoyant optimum policy allocates a unit of her acceptable product from product subgroup $\supplies_{\ell - 1}$.  

Based on the aforementioned instance construction, we numerically evaluate the performance \CUIB\ on instance $\hat\matchinginstance(20, 0.5, 0.3)$  with $n_0 = 500$, sufficiently large $\inventory$ and obtain a competitive ratio upper bound of 0.52966.






\xhdr{Analyzing \UDIB:} Consider an instance $\bar\matchinginstance(\epsilon)$ with $2$ products. Product 1 has price per unit $\reward_1 \triangleq 1$ and a large enough initial inventory $\inventory_1 \triangleq \inventory$. Product 2 has price per unit $\reward_2 \triangleq 1 - \epsilon$ and infinite initial inventory $\inventory_2 \triangleq \infty$. There are $T \triangleq \inventory + 2\inventory^2$ time periods. At each time period $t\in\{\inventory + 1, \inventory + 3, \dots, T - 1\}$, a new unit of product $1$ is added due to exogenous inventory shock. 

For every time period $t \in[\inventory]$, a consumer who only accepts product $1$ arrives. For every time period $t\in\{\inventory + 1, \inventory + 3,\dots, T - 1\}$, a consumer who accepts both products $1$ and $2$ arrives. For every time period $t\in \{\inventory + 2, \inventory + 4, \dots, T\}$, a consumer who only accepts product $1$ arrives.

The clairvoyant optimum policy allocates a unit of product $1$ to every consumer $t\in[t]\cup\{\inventory + 2, \inventory + 4, \dots, T\}$ and collect per unit price $\reward_1 = 1$. Meanwhile, it allocates a unit of product $2$ to every consumer $t\in \{\inventory + 1, \inventory + 3,\dots, T - 1\}$ and collect per unit price $\reward_2 = 1 - \epsilon$. Hence, the total revenue of the clairvoyant optimum policy is $T - \frac{T - \inventory}{2}\epsilon = \inventory + 2\inventory^2 - \inventory^2\epsilon$.

On the other end, \UDIB~ allocates a unit of product $1$ to every consumer $t\in[t]\cup\{\inventory + 1, \inventory + 3,\dots, T - 1\}$, and allocates nothing to every consumer $t\in\{\inventory + 2, \inventory + 4, \dots, T\}$. Consequently, the total revenue of the algorithm is $\inventory + \frac{T - \inventory}{2} = \inventory + \inventory^2$.

Putting two pieces together, the competitive ratio of the algorithm on this constructed instance is $\frac{\inventory + \inventory^2}{\inventory + 2\inventory^2 - \inventory^2\epsilon}$ which converges to $\frac{1}{2}$ as $\epsilon$ goes to zero and $\inventory$ goes to infinity.
\hfill\halmos    
\end{proof}


==> Paper/apx-prelim.tex <==

\label{apx:prelim}

\lemrelax*
\begin{proof}{\textsl{Proof.}}
Let $\event_{\indexnew,t}
(\boldsymbol\choice, \boldsymbol\replen)$ be the event that 
clairvoyant benchmark offers 
unit-specified assortment $\indexnew$ at time $t$ for a given 
sequence $\boldsymbol\choice = \{\choice_t\}_{t\in[\totaltime]},
\boldsymbol \replen = \{\repleni\}_{i\in[n],t\in[\totaltime]}$. 
As clairvoyant benchmark is inventory feasible 
for any sample path of products-units set selected by consumers 
$\boldsymbol\selectedproduct=\selectedproducts$, 
for all $i \in [n],
\ k\in [\finalinventory_i],
\ t \in [\addtime(i,k), \totaltime]$ we clearly have:
\begin{equation*}
\displaystyle\sum\nolimits_{\tpre = t}^{
\min\{t+\duration_i - 1, \totaltime\}}
	\displaystyle\sum\nolimits_{\indexnew \in \indexset(\tpre)}
    \indicator{(i,k) \in \selectedproduct_{\tpre}}\,
	\indicator{\event_{\indexnew,\tpre}
(\boldsymbol\choice, \boldsymbol\replen)} \leq 1
\end{equation*}
Condition on the platform offers unit-specified 
assortment $\indexnew$
to 
a consumer $\tpre$ with type $\choice_{\tpre}$, 
the probability 
that consumer $\tpre$ select unit $k$ of product $i$ is
$\choice_{\tpre}(\indexnew,i)$.
Therefore,
$\curalloc=\prob{
\event_{\indexnew,t}(\boldsymbol\choice, \boldsymbol\replen)
\condition 
\boldsymbol\choice, \boldsymbol\replen
}$ 
results in a feasible assignment for \ref{eq:exante-adversarial}. 
Moreover, 
the objective value under this assignment 
will be equal to the expected revenue 
of the clairvoyant benchmark, which finishes the proof.
\end{proof}

==> Paper/interval-assignment-old.tex <==
We now prove the key technical lemma about Interval Assignment Problem (\Cref{lem:IAP}) with an algorithmic proof. In particular, we first argue that \Cref{alg:interval assignment} terminates and generates an assignment. Then, we verify \hyperref[lem:IAP]{\LocalDominance}, \hyperref[lem:IAP]{\GlobalDominance} and \hyperref[lem:IAP]{\PartitionMonotonicity} in \Cref{lem:IAP} separately.



\begin{proof}{\textsl{Proof of \Cref{lem:IAP}}.}
In each iteration of the while loop, \Cref{alg:interval assignment} determines the assignment for one remaining interval and then removes it from $\remainingcontain$. Thus, the algorithm terminates and outputs an assignment $\{\assign_1, \dots, \assign_s\}$ as desired. We next verify that this assignment satisfies all three desired properties in the statement of the lemma.


\input{Paper/alg-IAP}

\noindent\emph{(\rom{1}) \hyperref[lem:IAP]{\LocalDominance}:}
For each interval $i \in [s]$, consider $j_1, j_2, \dots \in \contain_i$ in the order in which they are removed from the algorithm: for the $k$-th removed interval $j_k \in \contain_i$, at that time the cardinality $\remainingcontainni$ is $\containni - k + 1$, which guarantees that $\assign_{j_k}$ is at least $\containni - k + 1$ by construction. Thus, \hyperref[lem:IAP]{\LocalDominance} is satisfied.


\noindent\emph{(\rom{2}) \hyperref[lem:IAP]{\GlobalDominance}:}
We verify this property by the following induction argument. Consider the reverse order of intervals removed from the remaining interval set $\remaining$ in the algorithm, i.e., we set $\remaining = \emptyset$ as the base case and then add intervals back to $\remaining$ in the reverse order in which they have been removed in the algorithm. Our induction hypothesis is that restricting to intervals in $\remaining$, \hyperref[lem:IAP]{\GlobalDominance} holds, i.e., for any decreasing and concave function $\bar\pen$, 
\begin{align}
\label{eq:global dominance}
\sum\nolimits_{i\in \remaining} \bar\pen(\assign_i) \geq \sum\nolimits_{i \in \remaining} \bar\pen(\remainingcontainni).
\end{align}

\noindent\textbullet\ \emph{Base Case ($\remaining = \emptyset$):} In this case, the induction hypothesis holds trivially.

\noindent\textbullet\ \emph{Inductive Step:}  Suppose the induction hypothesis holds before we add interval $i$ with assignment~$\assign_{i}$ back to $\remaining$. Let $m \triangleq \assign_{i} - 1$. To make it clear, let $\remaining$ to be the remaining interval set before we add interval $i$, and $\remaining'$ to be the remaining interval set after we add interval $i$, i.e., $\remaining' = \remaining \cup\{i\}$. Next we analyze the increment of both sides in inequality~\eqref{eq:global dominance} after we add interval $i$ into $\remaining$. The left-hand side of inequality~\eqref{eq:global dominance} increases by $\bar\pen(m + 1)$. For the right-hand side, since $\assign_i = m + 1$, there exist $m$ intervals $j_1, j_2, \dots j_m \in \remaining$ which cover position $a_{\pmother_i}$, and $i < j_k$ (otherwise, $j_k$ should be removed earlier than $i$ in the algorithm) for all $k\in[m]$. This implies that interval $i$ covers position $a_{j_k}$ for all $k \in[m]$. Without loss of generality, we assume $j_1 < j_2 < \dots < j_m$. We have $|\remainingcontain_{j_k}|\geq k$ for all $k\in[m]$. Hence, after adding interval $i$ into $\remaining$, the right-hand side of inequality~\eqref{eq:global dominance} increases by 
\begin{align*} 
&\bar\pen(|\contain_i^{\remaining'}|) + 
\sum\nolimits_{j\in \remaining}
\left(
\bar\pen(|\contain_{j}^{\remaining'}|) - 
\bar\pen(|\contain_{j}^{\remaining}|)
\right) 
\overset{(a)}{\leq} \bar\pen(|\contain_i^{\remaining'}|) + 
\sum\nolimits_{k\in[m]}
\left(
\bar\pen(|\contain_{j_k}^{\remaining'}|) - 
\bar\pen(|\remainingcontain_{j_k}|)
\right) \\
\overset{(b)}{=}{}&
\bar\pen(|\contain_i^{\remaining'}|) + 
\sum\nolimits_{k\in[m]}
\left(\bar\pen(|\remainingcontain_{j_k}| + 1) - 
\bar\pen(|\remainingcontain_{j_k}|)\right) 
\overset{(c)}{\leq} 
\bar\pen(1) + 
\sum\nolimits_{k \in [m]}
(
\bar\pen(k + 1) - \bar\pen(k)
)
= \bar\pen(m + 1)
\end{align*}
where inequality~(a) holds since $|\contain_{j_k}^{\remaining'}| \geq |\contain_{j_k}^{\remaining}|$ and $\bar\pen$ is decreasing; equality~(b) holds since $|\contain_{j_k}^{\remaining'}|  = |\remainingcontain_{j_k}| + 1$ by construction; and inequality~(c) holds since $\bar\pen$ is decreasing, concave and $|\remainingcontain_{j_k}|\geq k$ for all $k\in[m]$. Applying the induction hypothesis (before we add interval $i$), the inductive statement (after we add interval $i$) holds, which finishes the induction as desired.
% \vspace{-4mm}
\input{Paper/alg-IAP-partition}
% \vspace{-mm}
\noindent\emph{(\rom{3}) \hyperref[lem:IAP]{\PartitionMonotonicity}:}
We first introduce the following two claims: (a) for each interval $i\in[s]$, there is at most one interval $j$ such that $\pfather_j = i$; (b) for each interval $i\in[s]$ with $\assign_i > 1$, $\pfather_i \not= -1$. Note that claims (a) and (b) together imply that $\{\pfather_1, \dots, \pfather_s\}$ 
defines a partition which satisfies \hyperref[lem:IAP]{\PartitionMonotonicity} from \Cref{alg:partition monotonicity construction}.

Next, we show claim (a) and claim (b) separately. We show claim (a) by contradiction. Suppose there exists interval $i$, $j_1$ and $j_2$ such that $\pfather_{j_1} = \pfather_{j_2} = i$. By the construction of \Cref{alg:interval assignment}, $\assign_{j_1} = \assign_{j_2} = \assign_i + 1$. Now, consider case by case.



\noindent\textbullet\ \emph{Case 1 ($i < j_1$ or $i < j_2$):} W.L.O.G., we assume $i < j_1$,
and the case $i < j_2$ is symmetric.
By the construction of \Cref{alg:interval assignment},
$\pfather_{j_1} = i$ implies 
$i \in \contain_{\pmother_{j_1}}$. 
This leads to a contradiction because if $i < j_1$, the interval $i$ should be removed earlier than the interval $j_1$ in \Cref{alg:interval assignment}
which implies $\assign_i \geq \assign_{j_1}$.

\noindent\textbullet\ 
\emph{Case2 ($j_1, j_2 < i$):}

\hspace{5mm}\noindent\textbullet\ 
\emph{Case 2a ($\pmother_{j_1} < \pmother_{j_2}$ or $\pmother_{j_2} < \pmother_{j_1}$):}
W.L.O.G., we assume $\pmother_{j_1} < \pmother_{j_2}$ ($\pmother_{j_2} < \pmother_{j_1}$ is similar):

\hspace{10mm}\noindent\textbullet\ \
\emph{Case 2a1 (interval $j_1$ is removed before interval $j_2$):}
In this case, consider the moment 
when \Cref{alg:interval assignment} removes $j_1$ due to interval $\pmother_{j_1}$.
By the construction of \Cref{alg:interval assignment}, since $j_1$ is removed before $j_2$,
it implies
$|\remainingcontain_{\pmother_{j_1}}| > |\remainingcontain_{\pmother_{j_2}}|$.
Thus,
$\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
contradiction.

\hspace{10mm}\noindent\textbullet\ \
\emph{Case 2a2 (interval $j_2$ is removed before interval $j_1$):}
In this case, consider the moment 
when \Cref{alg:interval assignment} remove $j_2$ due to interval $\pmother_{j_2}$.
Notice that interval $j_2$ also covers position $a_{\pmother_{j_1}}$,
i.e., $j_2 \in \contain_{\pmother_{j_1}}$.
By the construction of \Cref{alg:interval assignment}, since $j_2$ is removed before $j_1$,
it implies
$|\remainingcontain_{\pmother_{j_1}}|  \leq |\remainingcontain_{\pmother_{j_2}}|$.
Thus, once \Cref{alg:interval assignment} removed $j_2$, 
$|\contain_{\pmother_{j_1}}^{\remaining/\{j_2\}}|$ (which is an upper bound
of $\assign_{j_1}$) 
becomes strictly smaller than 
$|\remainingcontain_{\pmother_{j_2}}|$ (which is equal to $\assign_{j_2}$), 
contradiction.


\hspace{5mm}\noindent\textbullet\ 
\emph{Case 2b ($\pmother_{j_1} = \pmother_{j_2}$):}
Without loss of generality, we assume interval $j_1$ is removed before interval $j_2$,
and the case where interval $j_2$ is removed before interval $j_1$ is 
symmetric.
Let $\pmother^* = \pmother_{j_1} = \pmother_{j_2}$. Consider the moment
when \Cref{alg:interval assignment} removes $j_1$ due to $\pmother^*$.
By the construction of \Cref{alg:interval assignment},
$\assign_{j_1} = 
|\remainingcontain_{\pmother^*}|$
and $\assign_{j_2} \leq |\contain_{\pmother^*}^{\remaining/\{j_1\}}|
= |\remainingcontain_{\pmother^*}| - 1$.
Thus, $\assign_{j_1}>\assign_{j_2}$,
which is a contradiction.

\vspace{1.5mm}

We show claim (b) as follows. For any interval $i$ with $\assign_i > 1$, consider the next removed interval $j$ among $\contain_{\pmother_i}$ after \Cref{alg:interval assignment} removes interval $i$. It is sufficient to show $\assign_j = \assign_i - 1$, which implies that \Cref{alg:interval assignment} sets $\pfather_i = j$ when it removes interval $j$. Since $j$ is the next interval removed among $\contain_{\pmother_i}$ after interval $i$, we have $\assign_i - 1\leq \assign_j \leq \assign_i$. To show $\assign_j < \assign_i$, we use the proof by contradiction. Suppose $\assign_j = \assign_i$. If $i\in\contain_{\pmother_j}$, then at the moment when \Cref{alg:interval assignment} removes $i$, we have $\assign_i = |\contain_{\pmother_i}^{\remaining}|\geq|\contain_{\pmother_j}^{\remaining}| \geq \assign_j + 1 = \assign_i + 1$, which is a contradiction. If $i \not\in \contain_{\pmother_j}$, since $i < j$, we have mapping $\pmother_i < \pmother_j$ and at the moment when \Cref{alg:interval assignment} removes $i$, $|\contain_{\pmother_i}^\remaining| = \assign_i =\assign_j  \leq  \contain_{\pmother_j}^\remaining|$, a contradiction.
\hfill\halmos
\end{proof}

==> figs/fig-bin-structure.tex <==
\begin{tikzpicture}[scale = 0.35,
every node/.style={scale=0.5}]


\begin{scope}[thick]
\draw (0,0) -- (3, 0) -- (3, 10) -- (0, 10) --(0,0);

\draw (4,0) -- (7, 0) -- (7, 4) -- (4, 4) --(4,0);

\draw (8,0) -- (11, 0) -- (11, 10.5) -- (8, 10.5) --(8,0);
\draw (12, 0) -- (15, 0) -- (15, 5) -- (12, 5) -- (12,0);
\draw (16, 0) -- (19, 0) -- (19, 2) -- (16, 2) -- (16,0);
\end{scope}

\draw [thick, dashed, color=gray] (-0.4, 3.5) -- (19.4, 3.5);
\draw(-1, 3.5) node {$\gamma\inventory_i$};

\draw [thick, dashed, color=gray] (-0.4, 8) -- (19.4, 8);
\draw(-1, 8) node {$\inventory_i$};

\draw (1.5, -0.5) node {$\batch_{i,1}$};
\draw (5.5, -0.5) node {$\batch_{i,2}$};
\draw (9.5, -0.5) node {$\batch_{i,3}$};
\draw (13.5, -0.5) node {$\batch_{i,4}$};
\draw (17.5, -0.5) node {$\batch_{i,5}$};

\draw [thick, dotted,color=gray](-0.4, -1) -- (-0.4, 12) -- (15.4, 12) -- (15.4, -1) 
-- (-0.4, -1);

\draw [thick, dotted,color=gray] (15.6, 12) -- (19.4, 12) -- (19.4, -1) 
-- (15.6, -1)
--
(15.6, 12);
\draw (7.5, 11.5) node {\emph{ready}};

\draw (17.5, 11.5) node {\emph{batching}};
\end{tikzpicture}

==> figs/fig-binTilde-structure.tex <==
\begin{tikzpicture}[scale = 0.35,
every node/.style={scale=0.5}]


\fill[red!10!white] (-0.5, -1) -- (-0.5, 10.5) -- (3.7, 10.5) -- (3.7, 3.5) 
-- (7.3, 3.5) -- (7.3, -1) -- (-0.5, -1);


\fill[yellow!10!white] (3.7, 3.5) -- (3.7, 4.5) -- (7.7, 4.5) -- (7.7, 3.5) 
-- (11.3, 3.5) -- (11.3, -1) -- (7.3, -1)
-- (7.3,3.5) -- (3.7, 3.5);

\fill[blue!10!white] (7.7, 3.5) -- (7.7, 11) -- (11.7, 11) -- (11.7, 3.5) 
-- (15.3, 3.5) -- (15.3, -1) -- (11.3, -1)
-- (11.3, 3.5) -- (7.7, 3.5);

\fill[green!10!white] (11.7, 3.5) -- (11.7, 5.5) -- (15.7, 5.5) -- (15.7, 2.5) 
-- (19.3, 2.5) -- (19.3, -1) -- (15.3, -1)
-- (15.3,3.5) -- (11.7, 3.5);


\begin{scope}[thick]
\draw (0,0) -- (3, 0) -- (3, 10) -- (0, 10) --(0,0);

\draw (4,0) -- (7, 0) -- (7, 4) -- (4, 4) --(4,0);

\draw (8,0) -- (11, 0) -- (11, 10.5) -- (8, 10.5) --(8,0);
\draw (12, 0) -- (15, 0) -- (15, 5) -- (12, 5) -- (12,0);
\draw (16, 0) -- (19, 0) -- (19, 2) -- (16, 2) -- (16,0);
\end{scope}

\draw [thick, dotted, color=gray] (-0.4, 3.5) -- (3.5, 3.5);
\draw(-1, 3.5) node {$\gamma\inventory_i$};

\draw [thick, dotted, color=gray] (-0.4, 8) -- (19.4, 8);
\draw(-1, 8) node {$\inventory_i$};

\draw (3, -0.5) node {$\batchTilde_{i}^{1}$};
\draw (9.5, -0.5) node {$\batchTilde_{i}^{2}$};
\draw (13.5, -0.5) node {$\batchTilde_{i}^{3}$};
\draw (17.5, -0.5) node {$\batchTilde_{i}^{4}$};

\draw [line width=2pt, dotted,color=gray]
(-0.5, -1) -- (-0.5, 10.5) -- (3.7, 10.5) -- (3.7, 3.5) 
-- (7.3, 3.5) -- (7.3, -1) -- (-0.5, -1);

\draw [line width=2pt, dotted,color=gray]
(3.7, 4.5) -- (7.7, 4.5)
--
(7.7, 3.5) -- (11.3, 3.5)
--
(11.3, -1) -- (7.3, - 1);

\draw [line width=2pt, dotted,color=gray]
(7.7, 4.5) -- (7.7, 11)
-- (11.7, 11)
--
(11.7, 3.5) -- (15.3, 3.5)
--
(15.3, - 1) -- (11.3, -1);

\draw [line width=2pt, dotted,color=gray]
(11.7, 5.5)
--
(15.7, 5.5) -- (15.7, 2.5)
--
(19.3, 2.5) -- (19.3, - 1) -- (15.3, -1);



\end{tikzpicture}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
